A Note on the Post-Quantum Security of (Ring) Signatures

This work revisits the security of classical signatures and ring signatures in a quantum world. For (ordinary) signatures, we focus on the arguably preferable security notion of blind-unforgeability recently proposed by Alagic et al. (Eurocrypt'20). We present two short signature schemes achieving this notion: one is in the quantum random oracle model, assuming quantum hardness of SIS; and the other is in the plain model, assuming quantum hardness of LWE with super-polynomial modulus. Prior to this work, the only known blind-unforgeable schemes are Lamport's one-time signature and the Winternitz one-time signature, and both of them are in the quantum random oracle model. For ring signatures, the recent work by Chatterjee et al. (Crypto'21) proposes a definition trying to capture adversaries with quantum access to the signer. However, it is unclear if their definition, when restricted to the classical world, is as strong as the standard security notion for ring signatures. They also present a construction that only partially achieves (even) this seeming weak definition, in the sense that the adversary can only conduct superposition attacks over the messages, but not the rings. We propose a new definition that does not suffer from the above issue. Our definition is an analog to the blind-unforgeability in the ring signature setting. Moreover, assuming the quantum hardness of LWE, we construct a compiler converting any blind-unforgeable (ordinary) signatures to a ring signature satisfying our definition.

==> sections/Ring-Sig.tex <==
%!TEX root=../main.tex
\section{Post-Quantum (Compact) Ring Signatures}
\subsection{Definitions}\label{sec:PQ-ring-sig:def}
\subsubsection{Classical Ring Signatures} 
We start by recalling the classical definition of ring signatures \cite{TCC:BenKatMor06,EC:BDHKS19}.

\begin{definition}[Ring Signature]
	\label{def:classical:ring-signature}
	A ring signature scheme \algo{RS} is described by a triple of PPT algorithms \algo{(Gen,Sign,Verify)} such that:
	\begin{itemize}
		
		\item {\bf $\Gen(1^\lambda,N)$:} on input a security parameter $1^\lambda$ and a super-polynomial\footnote{The $N$ has to be super-polynomial to support rings of {\em arbitrary} polynomial size.} $N$ (e.g., $N = 2^{\log^2\secpar}$) specifying the maximum number of members in a ring, output a verification and signing key pair $\algo{(VK,SK)}$. 
		
		\item {\bf $\algo{Sign}(\SK,\Ring, m)$:} given a secret key \SK, a message $m \in \mathcal{M}_\lambda$, and a list of verification keys (interpreted as a ring) $\algo{R = (VK_1,\cdots,VK_\ell)}$ as input, and outputs a signature $\Sigma$. 
		
		\item {\bf $\algo{Verify}(\Ring,m,\Sigma)$:} given a ring $\algo{R = (VK_1,\dots,VK_\ell)}$, message $m \in \mathcal{M}_\lambda$ and a signature $\Sigma$ as input, outputs either 0 (rejecting) or 1 (accepting).  
	\end{itemize}
	These algorithms satisfy the following requirements:  
	\begin{enumerate}
		\item {\bf Completeness:} for all $\lambda \in \Naturals$, $\ell \le N$, $i^* \in [\ell]$, and $m \in \mathcal{M}_\lambda$, it holds that $\forall i \in [\ell]$ $(\VK_i,\SK_i) \gets \Gen(1^\lambda,N)$ and $\Sigma \gets \algo{Sign}(\SK_{i^*},\Ring,m)$ where $\algo{R = (VK_1,\dots,VK_\ell)}$, we have $\Pr[\algo{RS.Verify}(\Ring,m,\Sigma) = 1] = 1$, 
		where the probability is taken over the random coins used by $\Gen$ and $\algo{Sign}$.
		
		
		\item {\bf Anonymity:} For any $Q = \poly(\secpar)$ and any PPT adversary $\Adv$, it holds w.r.t.\ \Cref{expr:classical-anonymity} that 
		$\algo{Adv}_\textsc{Anon}^{\secpar, Q}(\Adv) \coloneqq \big|\Pr\big[\algo{Exp}_\textsc{Anon}^{\secpar, Q}(\Adv) = 1\big] - 1/2\big| \le \negl(\secpar)$.
		\begin{ExperimentBox}[label={expr:classical-anonymity}]{Classical Anonymity \textnormal{$\algo{Exp}_\textsc{Anon}^{\secpar, Q}(\Adv)$}}
		\begin{enumerate}[label={\arabic*.},leftmargin=*,itemsep=0em]
			\item 
			For each $i \in [Q]$, the challenger generates key pairs $(\VK_i,\SK_i) \gets \Gen(1^\lambda, N;r_i)$. It sends $\Set{(\VK_i, \SK_i, r_i)}_{i\in [Q]}$ to $\Adv$;
			\item 
			$\Adv$ sends a challenge to the challenger of the form $(i_0,i_1,\Ring,m)$.\footnote{We stress that $\Ring$ might contain keys that are not generated by the challenger in the previous step. In particular, it might contain maliciously generated keys.} The challenger checks if $\VK_{i_0} \in \Ring$ and $\VK_{i_1} \in \Ring$. If so, it samples a uniform bit $b$, computes $\Sigma \gets \algo{Sign}(\SK_{i_b},\Ring,m)$, and sends $\Sigma$ to $\Adv$. 
			\item 
			$\Adv$ outputs a guess $b'$. If $b' = b$, the experiment outputs 1, otherwise 0.
		\end{enumerate}
		\end{ExperimentBox}

		\item {\bf Unforgeability:} for any $Q=\poly(\lambda)$ and any PPT adversary $\Adv$, it holds w.r.t.\ \Cref{expr:classical:unforgeability} that 
		$\algo{Adv}_\textsc{Unf}^{\secpar,  Q}(\Adv) \coloneqq \Pr\big[\algo{Exp}_\textsc{Unf}^{\secpar,  Q}(\Adv) = 1\big] \le \negl(\secpar)$.

		\begin{ExperimentBox}[label={expr:classical:unforgeability}]{Classical Unforgeability \textnormal{$\algo{Exp}_\textsc{Unf}^{\secpar, Q}(\Adv)$}}
		\begin{enumerate}[label={\arabic*.},leftmargin=*,itemsep=0em]
			\item For each $i \in [Q]$, the challenger generates $(\VK_i,\SK_i) \gets \Gen(1^\lambda,N;r_i)$, and stores these key pairs along with their corresponding randomness. It then sets $\mathcal{VK} = \Set{\VK_1,\dots,\VK_Q}$ and initializes a set $\mathcal{C} = \emptyset$. 
			\item The challenger sends $\mathcal{VK}$ to $\Adv$. 
			\item $\Adv$ can make polynomially-many queries of the following tow types: 
			\begin{itemize}[leftmargin=*,itemsep=0em,topsep=0em]
			\item {\bf Corruption query $(\mathsf{corrupt},i)$:} The challenger adds $\VK_i$ to the set $\mathcal{C}$ and returns the randomness $r_i$ to \Adv. 
			\item {\bf Signing query $(\algo{sign},i,\Ring,m)$:} The challenger first checks if $\VK_i \in \Ring$. If so, it computes $\Sigma \gets \algo{Sign}(\SK_i,\Ring,m)$ and returns $\Sigma$ to \Adv. It also keeps a list of all such queries made by \Adv. 
			\end{itemize}   
			\item Finally, $\Adv$ outputs a tuple $(\Ring^*, m^*, \Sigma^*)$. The challenger checks if: 
			\begin{itemize}[leftmargin=*,itemsep=0em,topsep=0em]
				\item $\Ring^* \subseteq \mathcal{VK \setminus C}$,
				\item $\Adv$ never made a signing query of the form $(\algo{sign},\cdot,\Ring^*, m^*)$, {\bf and}
				\item $\algo{Verify}(\Ring^*,m^*,\Sigma^*) = 1$.
			\end{itemize}
			If so, the experiment outputs 1; otherwise, it outputs 0.
		\end{enumerate}
		\end{ExperimentBox}		
		\item {\bf Compactness (Optional):} 
		the scheme is said to be {\em compact} if the size of a signature is upper-bounded by a polynomial in $\lambda$ and $\log N$.
	\end{enumerate}
\end{definition}
We mention that the unforgeability and anonymity properties defined in \autoref{def:classical:ring-signature} correspond respectively to the notions of \emph{unforgeability with insider corruption} and \emph{anonymity with respect to full key exposure} presented in \cite{TCC:BenKatMor06}.



\subsubsection{Defining Post-Quantum Security}
We aim to build a classical ring signature scheme that can protect against adversaries making superposition queries to the singing oracle. Formalizing the security requirements in this scenario is non-trivial. An initial step toward this direction has been taken in \cite{C:CGHKLMPS21}. But their definition has certain restrictions (discussed below). In the following, we develop a new definition built on top of that from \cite{C:CGHKLMPS21}.

\para{Post-Quantum Anonymity.} Recall that in the classical anonymity game (\Cref{expr:classical-anonymity}), the adversary's query is of the quadruple $(i_0,i_1,\Ring,m)$. To define post-quantum anonymity, a natural attempt is to allow the adversary to send a superposition of this quadruple, and to let the challenger respond using the following unitary mapping\footnote{Of course, the challenger also needs to check if $\VK_{i_0} \in \Ring$ and $\VK_{i_1} \in \Ring$. But we can safely ignore this for our current discussion.}:
$$\sum_{i_0,i_1,\Ring,m,t} \psi_{i_0, i_1, \Ring, m,  t}\ket{i_0, i_1, \Ring, m, t} \mapsto \sum_{i_0,i_1,\Ring,m,t} \psi_{i_0, i_1, \Ring, m, t}\ket{i_0, i_1, \Ring, m, t \oplus \Sign(\SK_{i_b}, m, \Ring;r)}.$$ 
However, as observed in \cite{C:CGHKLMPS21}, this will lead to a unsatisfiable definition due to an attack from \cite{C:BonZha13}. Roughly speaking, the adversary could use classical values for $\Ring$, $m$, and $i_1$, but she puts a uniform superposition of all valid identities in the register for $i_0$. After the challenger's signing operation, observe that if $b = 0$, the last register will contain  signatures in superposition (as $i_0$ is in superposition); if $b = 1$, it will contain a classical signature (as $i_1$ is classical). These two cases can be efficiently distinguished by means of a Fourier transform on the $i_0$'s register followed by a measurement. Therefore, to obtain an achievable notion, we should not allow superpositions over $(i_0, i_1)$. 

Now, $\Adv$ only has the choice to put superpositions over $\Ring$ and $m$. The definition in \cite{C:CGHKLMPS21} further forbids $\Adv$ from putting superposition over $\Ring$. But this is only because they did not know how to prove security if superposition attacks on $\Ring$ is allowed. Indeed, they left it as an open problem to construct a scheme that protects against superposition attacks on $\Ring$. We in this work solve this problem. So, our definition allows superposition attacks on both $\Ring$ and $m$.
\begin{definition}[Post-Quantum Anonymity]
\label{def:pq:anonymity}
Consider a triple of PPT algorithms $\RS = (\algo{Gen}, \Sign, \Verify)$ that satisfies the same syntax as in \Cref{def:classical:ring-signature}. $\RS$ achieves post-quantum anonymity if for any $Q=\poly(\lambda)$ and any QPT adversary $\Adv$, it holds w.r.t.\ \Cref{expr:pq:anonymity} that 
		$$\algo{PQAdv}_\textsc{Anon}^{\secpar,Q}(\Adv) \coloneqq \big|\Pr\big[\algo{PQExp}_\textsc{Anon}^{\secpar,Q}(\Adv) = 1\big] - 1/2\big| \le \negl(\secpar).$$
\begin{ExperimentBox}[label={expr:pq:anonymity}]{Post-Quantum Anonymity \textnormal{$\algo{PQExp}_\textsc{Anon}^{\secpar,Q}(\Adv)$}}
\begin{enumerate}[leftmargin=*,itemsep=0em]
\item 
For each $i \in [Q]$, the challenger generates key pairs $(\VK_i,\SK_i) \leftarrow \RS.\algo{Gen}(1^\SecPar, N;r_i)$. The challenger sends $\Set{(\VK_i, \SK_i, r_i)}_{i\in [Q]}$ to $\Adv$;
\item
$\Adv$ sends $(i_0, i_1)$ to the challenger, where both $i_0$ and $i_1$ are in $[Q]$;
\item
$\Adv$'s challenge query is allowed to be a superposition of rings {\em and} messages. The challenger picks a random bit $b$ and a random string $r$. It signs the message using $\SK_{i_b}$ and randomness $r$, while making sure that $\VK_{i_0}$ and $\VK_{i_1}$ are indeed in the ring specified by $\Adv$. Formally, the challenger implements the following mapping:
$$\sum_{\Ring, m, t}\psi_{\Ring, m, t} \ket{ \Ring, m, t} \mapsto \sum_{\Ring, m, t}\psi_{\Ring, m, t} \ket{\Ring, m, t\xor f(\Ring, m)},$$
where
$f(\Ring, m) \coloneqq
\begin{cases}
\RS.\Sign(\SK_{i_b}, R, m;r) & \text{if}~\VK_{i_0}, \VK_{i_1} \in R \\
\bot & \text{otherwise}
\end{cases}
$.
\item 
$\Adv$ outputs a guess $b'$. If $b' = b$, the experiment outputs 1, otherwise 0.
\end{enumerate}
\end{ExperimentBox}
\end{definition}


\para{Post-Quantum Unforgeability.} In the classical unforgeability game (\Cref{expr:classical:unforgeability}), $\Adv$ can make both {\sf corrupt} queries and {\sf sign} queries. \xiao{As mentioned in the intro/tech-overview,} we do not consider quantum {\sf corrupt} queries, because it is unclear what it means to ``corrupt a superposition of all the ring members''. For the same reason, we do not consider superposition attacks over the identity in $\Adv$'s {\sf sign} queries, and only allows the ring and the message to be in superposition. 
\begin{xiaoenv}{Superpositions for Unforgeability Game}
We need to argue the requirement of classical identity properly in the intro. Also, for {\sf sign} queries, mention the setting that a single user is corrupted and enforced into quantum behaviors. However, this user only knows his own key; even if he is quantum now, he can only sign with his own key.
\end{xiaoenv}
We remark that in the unforgeability game, \cite{C:CGHKLMPS21} does not allow superpositions over the ring. Instead of a definitional issue, this is again only because they does not know how to prove the security of their construction if superposition attacks on the ring is allowed. In contrast, our construction can be proven secure against such attacks; thus, this restriction is removed from our definition.

In the post-quantum unforgeability game, extra caution is needed to define ``valid'' forgeries. \cite{C:CGHKLMPS21} follows the ``one-more forgery'' definition \xiao{as mentioned in intro/tech-overview/prelim?}. Concretely, it is required that the adversary cannot produce $(\mathsf{sq} + 1)$ valid signatures by making only $\mathsf{sq}$ quantum {\sf sign} queries.

However, in contrast to ordinary signatures, there is one caveat unique to the ring setting. Recall in \Cref{expr:classical:unforgeability} that the adversary's forgery contains a ring $\Ring^*$. This forgery will be considered as valid only if $\Ring^*$ consists of the uncorrupted members (i.e.\ $\Ring^* \subseteq \mathcal{VK}\setminus \mathcal{C}$). A natural generalization of the ``one-more forgery'' approach here is to require that, with $\mathsf{sq}$ quantum signing queries, adversary cannot produce $\mathsf{sq} + 1$ signatures, where all the rings are subsets of $\mathcal{VK}\setminus \mathcal{C}$. But this definition, {\em when restricted to the classical setting}, seems to be weaker than the standard unforgeability in \Cref{def:classical:ring-signature}.\footnote{This is in contrast to the case of ordinary signatures, where ``one-more'' unforgeability is equivalent to the standard existential unforgeability \cite{C:BonZha13}.} That is, in the classical setting, any $\RS$ satisfying the unforgeability in \Cref{def:classical:ring-signature} is also unforgeable w.r.t.\ the ``one-more'' definition; but the reverse direction is unclear. The reason is as follows. \xiao{check Rothit's writing..} To argue that ``one-more'' unforgeability is no weaker than \Cref{def:classical:ring-signature}, one needs to show how to convert a forger $\Adv_\textsc{euf}$ winning in \Cref{expr:classical:unforgeability} to another forger $\Adv_\textsc{om}$ winning in the (classical version of) ``one-more forgery'' game. Conceivably, $\Adv_\textsc{om}$ will run $\Adv_\textsc{euf}$ internally; thus, $\Adv_\textsc{om}$ will make no less {\sf sign} queries than $\Adv_\textsc{euf}$. Recall that $\Adv_\textsc{om}$ needs to forge one more signature than the total number of its queries.
 Also, crucially, all the ring signatures presented by $\Adv_\textsc{om}$ at the end must have {\em no} corrupted members in the accompanying ring. Now ideally one might imagine that we can simply use the queries made by $\Adv_\textsc{om}$ (which are really queries by $\Adv_\textsc{euf}$) to meet the ``one-more'' challenge; however, this is thwarted immediately due to the fact that $\Adv_\textsc{euf}$ has absolutely no obligation to make queries meeting this requirement, so even if the final forgery produced by $\Adv_\textsc{euf}$ is valid, our attempted reduction does not have any means to provide $\Adv_\textsc{om}$ with all the signatures it needs to win the ``one-more'' challenge (since not all of the queries can be reused). Indeed, it is not hard to find attacks that use this definitional gap to violate standard unforgeability, while being ruled out as a valid attack against ``one-more'' ring unforgeability. Contrast this with a comparison in the other direction: an adversary $\Adv_\textsc{om}$ for the ``one-more'' security definition is easily converted into a standard $\Adv_\textsc{euf}$ adversary since not all of the signatures output by $\Adv_\textsc{om}$ at the end can be queries (by the pigeonhole principle); $\Adv_\textsc{euf}$ simple outputs the one that is not. 
We remark however that this definitional gap between standard ring signature unforgeability and the ``one-more'' version may not be inherent; rather, we just do not know how to meet this gap. Our arguments here should not be interpreted as a proof showing that the former notion is strictly stronger than the latter. We leave it as an open question to either demonstrate a separation, or prove that the two are actually equivalent.

In this work, we present an alternative post-quantum unforgeability definition for ring signatures. Our idea is to extend the blind-unforgeability for ordinary signatures (\Cref{def:classical-BU-sig}) to the ring setting. We present this version in \Cref{def:pq:blind-unforgeability}. In contrast to the ``one-more'' unforgeability, we will show in \Cref{lem:euf-ring-sig:bu-ring-sig} that, when restricted to the classical setting, this blind-unforgeability for ring signatures is indeed equivalent to the standard existential unforgeability in \Cref{def:classical:ring-signature}.

\begin{definition}[Post-Quantum Blind-Unforgeability]
\label{def:pq:blind-unforgeability}
Consider a triple of PPT algorithms $\RS = (\algo{Gen}, \Sign, \Verify)$ that satisfies the same syntax as in \Cref{def:classical:ring-signature}. For any security parameter $\secpar$, let $\mathcal{R}_\secpar$ and $\mathcal{M}_\secpar$ denote the ring space and message space, respectively. $\RS$ achieves blind-unforgeability if for any $Q=\poly(\lambda)$ and any QPT adversary $\Adv$, it holds w.r.t.\ \Cref{expr:pq:blind-unforgeability} that 
		$$\algo{PQAdv}_\textsc{bu}^{\secpar,Q}(\Adv) \coloneqq \Pr\big[\algo{PQExp}_\textsc{bu}^{\secpar,Q}(\Adv) = 1\big] \le \negl(\secpar).$$ 
\begin{ExperimentBox}[label={expr:pq:blind-unforgeability}]{Post-Quantum Blind-Unforgeability \textnormal{$\algo{PQExp}_\textsc{bu}^{\secpar,Q}(\Adv)$}}
\begin{enumerate}[leftmargin=*,itemsep=0em]
	\item 
	$\Adv$ sends a constant $0\le \epsilon \le 1$ to the challenger;
			
	\item 
	For each $i \in [Q]$, the challenger generates $(\VK_i,\SK_i) \gets \Gen(1^\lambda,N;r_i)$, and stores these key pairs along with their corresponding randomness. It then sets $\mathcal{VK} = \Set{\VK_1,\dots,\VK_Q}$ and initializes a set $\mathcal{C} = \emptyset$; The challenger sends $\mathcal{VK}$ to $\Adv$; 

	\item 
	The challenger defines a {\em blindset} $B^\RS_\varepsilon \subseteq 2^{\mathcal{R}_\secpar} \times \mathcal{M}_\SecPar$: every pair $(\Ring, m) \in 2^{\mathcal{R}_\secpar} \times \mathcal{M}_\SecPar$ is put in $B^\RS_\varepsilon$ with probability $\varepsilon$; 
	
	\item 
	$\Adv$ can make polynomially-many queries of the following two types:  
	\begin{itemize}[leftmargin=*,itemsep=0em,topsep=0em]
	\item 
	{\bf Classical corruption query $(\mathsf{corrupt},i)$:} The challenger adds $\VK_i$ to the set $\mathcal{C}$ and returns the randomness $r_i$ to \Adv. 
	\item 
	{\bf Quantum Signing query $(\algo{sign},i, \sum \psi_{\Ring, m, t}\ket{\Ring, m, t})$:} That is, $\Adv$ is allowed to query the signing oracle on some classical identity $i$ and  superpositions over rings and messages. The challenger samples a random string $r$ and performs the following mapping:
	$$\sum_{\Ring, m, t}\psi_{\Ring, m, t} \ket{\Ring, m, t} \mapsto \sum_{\Ring, m, t}\psi_{\Ring, m, t} \ket{\Ring, m, t\xor B^\RS_\epsilon f(\Ring, m)},$$
	where $B^\RS_\epsilon f(\Ring, m) \coloneqq
	\begin{cases}
	 \bot  & \text{if}~(\Ring, m) \in B^\RS_\epsilon \\
	f(\Ring, m) & \text{otherwise}
	\end{cases}
	$, and

	$f(\Ring, m) \coloneqq
	\begin{cases}
	\RS.\Sign(\SK_{i}, m, \Ring;r) & \text{if}~\VK_{i} \in \Ring \\
	\bot & \text{otherwise}
	\end{cases}
	$.
	\end{itemize}   
	\item Finally, $\Adv$ outputs a tuple $(\Ring^*, m^*, \Sigma^*)$. The challenger checks if: 
	\begin{itemize}[leftmargin=*,itemsep=0em,topsep=0em]
		\item $\Ring^* \subseteq \mathcal{VK \setminus C}$; 
		\item $\algo{Verify}(\Ring^*,m^*,\Sigma^*) = 1$; {\bf and}
		\item $(\Ring^*,m^*) \in B^\RS_\epsilon$.
	\end{itemize}
	If so, the experiment outputs 1; otherwise, it outputs 0.
\end{enumerate}
\end{ExperimentBox}
\end{definition}

\begin{lemma}\label{lem:euf-ring-sig:bu-ring-sig}
Restricted to (classical) QPT adversaries, a ring signature $\RS$ scheme is blind-unforgeable (\Cref{def:pq:blind-unforgeability}) if and only if it satisfies the unforgeability requirement in \Cref{def:classical:ring-signature}.
\end{lemma}
\begin{proof}
\xiao{This argument is very similar to \cite[Proposition 2]{EC:AMRS20}. It can go to the appendix.}

We show both sides of this equivalence in turn. In the following, by ``\Cref{expr:pq:blind-unforgeability}'', we refer to the classical version of \Cref{expr:pq:blind-unforgeability}, where the signing query is of the form $(\algo{sign}, i, \Ring, m)$ (i.e., $(\Ring, m)$ is classical), and is answered as $B^\RS_\epsilon f(\Ring, m)$.	

\subpara{Necessity ($\Leftarrow$).} Let us first show how blind-unforgeability implies  standard unforgeability (for classical settings). Assume we have an adversary $\Adv_\textsc{euf}$ that breaks standard unforgeability of $\RS$ as per  \Cref{def:classical:ring-signature}, i.e., in \Cref{expr:classical:unforgeability} it produces a forgery $(m^*,\Ring^*,\Sigma^*)$   that is valid with non-negligible probability $\nu(\SecPar)$. We show that this is easily converted into an adversary $\Adv_\textsc{bu}$ that wins \Cref{expr:pq:blind-unforgeability} with non-negligible probability as well. $\Adv_\textsc{bu}$ first sets $\epsilon(\SecPar)$ equal to $1/p(\SecPar)$, where $p(\secpar)$ denotes the (polynomial) running time of $\Adv_\textsc{euf}$ (the reasoning behind this choice will become clear very soon). It then simply forwards all the queries from $\Adv_\textsc{euf}$ to the blind-unforgeability challenger and the responses back to $\Adv_\textsc{euf}$. It also outputs whatever eventual forgery $\Adv_\textsc{euf}$ does. 

Let us consider the success probability of $\Adv_\textsc{bu}$. To start with, note that $\Adv_\textsc{euf}$ makes at most $p(\SecPar)$ many queries of the signing oracle. In each such query, we know that the 
$(\Ring, m)$ pair is in the blind set independently with probability $\epsilon$. Thus it is not in the blind set with probability $1-\epsilon$, and if so the query is answered properly. In turn, the probability that all the queries made are answered properly is then at least $(1-\epsilon)^{p(\SecPar)} \approx 1/e$ (this uses independence and $\epsilon = 1/p$), and so the probability that the forgery $(\Ring^*,m^*,\Sigma^*)$ is valid 
% (i.e., that $\Ring^*$ has no corrupted members, that $\algo{Verify}(\Ring^*,m^*,\Sigma^*) = 1$, and that $(\Ring^*,m^*)$ was not a previous query response) 
is then at least $(1-\epsilon)^{p(\SecPar)}\cdot\nu(\SecPar)$.
Finally, the forgery, even if successful, might lie in the blind set with probability $\epsilon$. So, the total probability that $\Adv_\textsc{euf}$ outputs a valid forgery {\em for the blind unforgeability game} is $(1-\epsilon)^{p(\SecPar)+1} \cdot \nu(\SecPar) \approx (1-\epsilon) \cdot \nu \cdot 1/e$, which is non-negligible since $\nu$ is non-negligible by assumption. Thus if $\Adv_\textsc{euf}$ violates standard ring signature unforgeability according to \Cref{def:classical:ring-signature}, then $\Adv_\textsc{bu}$ violates blind unforgeability for ring signatures according to \Cref{def:pq:blind-unforgeability}, as claimed. 

\subpara{Sufficiency ($\Rightarrow$).} Let us now turn to the other direction of the equivalence. Assume now that there exists an adversary $\Adv_\textsc{bu}$ that can break blind unforgeability of $\RS$, i.e., win \Cref{expr:pq:blind-unforgeability} with non-negligible probability $\nu(\secpar)$. We show an adversary $\Adv_\textsc{euf}$
that can win \Cref{expr:classical:unforgeability} with non-negligible probability. $\Adv_\textsc{euf}$ simply simulates \Cref{expr:pq:blind-unforgeability} for $\Adv_\textsc{bu}$ by answering oracle queries according to a locally-simulated version of $B^\RS_\epsilon f(\Ring,m)$. Concretely, the adversary $\Adv_\textsc{euf}$ proceeds by drawing a subset $B^\RS_\epsilon$ in the same manner as the challenger in \Cref{expr:pq:blind-unforgeability}  and answering queries made by $\Adv_\textsc{bu}$ according to $B^\RS_\epsilon f(\Ring,m)$. Two remarks are in order:
\begin{enumerate}
\item \label{item:euf-ring-sig:bu-ring-sig:remark1}
when $(\Ring, m) \in B^\RS_\secpar$, no signature needs to be done. That is, this query can be answered by $\Adv_\textsc{euf}$ without calling its own signing oracle;
\item
$\Adv_\textsc{euf}$ can construct the set $B^\RS_\epsilon$ by ``lazy sampling'', i.e., when a particular query $(\algo{sign}, i, \Ring, m)$ is made by $\Adv_\textsc{bu}$, 
whether $(\Ring, m) \in B^\RS_\epsilon$ and ``remembering'' this information in case the query is asked again.
\end{enumerate}
By assumption, $\Adv_\textsc{bu}$ produces a valid forgery. And it follows from \Cref{item:euf-ring-sig:bu-ring-sig:remark1} that this forgery must be on a point which was not queried by $\Adv_\textsc{euf}$, thus, also serving as a valid forgery for $\Adv_\textsc{euf}$'s game.
\iffalse
% Rohit's early argument w.r.t. strong EUF
	At this point we will consider the specific kind of ring signature scheme $\RS$ being used: specifically, whether this scheme has deterministic signatures or not. The overall idea is that $\Adv_\textsc{euf}$ will {\em locally} maintain and administer a blind set of size $\epsilon$ in its interation with $\Adv_\textsc{bu}$; but the exact manner on implementation will depend on what kind of scheme we use. The reason for this distinction will become clear from the following arguments. 

	Let us first consider the case of a deterministic ring signature $\RS$. In this case, we use essentially the same reduction as in the proof for \cite[Proposition 2]{EC:AMRS20} (they consider such an equivalence only for weak unforgeability - and this is precisely why their reduction works for the deterministic case). Namely, $\Adv_\textsc{euf}$ behaves as follows: it maintains a blind set with respect to messages and rings only. This is equivalent to maintaining a blind set over message, ring and signature triples for deterministic signatures. Whenever $\Adv_\textsc{bu}$ makes a query, $\Adv_\textsc{euf}$ adds this to the blind set with probability $\epsilon$. If the query gets added, $\Adv_\textsc{euf}$ simply replies with $\bot$ and does not forward the query to its own challenger. If not, it forwards the query and sends the response back to $\Adv_\textsc{bu}$ as per usual. Finally, $\Adv_\textsc{bu}$ outputs a forgery, say $(m^*,\Ring^*,\Sigma^*)$. With probability $\nu$, this is good enough to win the blind unforgeability challenge, implying that at the very least this forgery is not with respect to a message to a {\em successful} query. Indeed, nothing prevents $\Adv_\textsc{bu}$ from producing a forgery with respect to any message in $\Adv_\textsc{euf}$'s local blind set, including messages that it queried and recieved no response for. Crucially however, for these messages $\Adv_\textsc{euf}$ never queries its own oracle so even a forgery with respect to such messages suffices to win the standard unforgeability challenge. Thus $\Adv_\textsc{euf}$ can simply use the forgery output by $\Adv_\textsc{bu}$ in its own challenge, and win with probability at least $\nu(\SecPar)$. 

	Now we turn to the case of randomized ring signatures. For any such scheme $\RS$, since the signing algorithm $\RS.\Sign$ is randomized, we have the property that for any particular message $m$, ring $R$ and signing key $sk$ there are multiple signatures that are possible (depending on the randomness used by the signing algorithm). Define the guessing probability $\eta_{m,R,sk}$ to be the inverse of the number of possible signatures that can be generated by $\RS.\Sign$ given a choice of $(m,R,sk)$ (for most schemes, the number of signatures is usually independent of these choices and depends only on \SecPar). Further define $\eta_\RS = \mathsf{min}_{m,R,sk}\{\eta_{m,R,sk}\}$. By definition, we have that $\eta_\RS \leq 1/2$ for any randomized ring signature scheme $\RS$. We now describe the function of $\Adv_\textsc{euf}$ for this case. It forwards queries from $\Adv_\textsc{bu}$ and responses back to it, as before. Additionally, it maintains a local blind set (consisting of message, ring and signature triples). In contrast to the previous case, $\Adv_\textsc{euf}$ now queries its own (standard unforgeability) challenger on {\em all} queries $\Adv_\textsc{bu}$ makes. Upon obtaining the signature from the challenger, it adds the resulting triple to the blindset with probability $\epsilon$, and only returns $\bot$ to $\Adv_\textsc{bu}$ for such a query. Ultimately $\Adv_\textsc{bu}$ outputs a forgery $(m^*,\Ring^*,\sigma^*)$. This is guaranteed to be a valid forgery for the blinded unforgeability challenge (i.e., i.e., that $\Ring^*$ has no corrupted members, and that $\algo{Verify}(\Ring^*,m^*,\Sigma^*) = 1$) with probability at least $\nu$. 

	Let us consider two possibilities. Either the forgery $(m^*,\Ring^*,\sigma^*)$ was not queried by $\Adv_\textsc{euf}$ before, in which case it can simply use this forgery and win the standard unforgeability game. Otherwise, $\Adv_\textsc{bu}$ indeed asked for a signature with respect to $(m^*,\Ring^*)$ and obtained no response. In this case, $\Adv_\textsc{bu}$ may have output a signature $\Sigma^*$, and correspondingly $\Adv_\textsc{euf}$ recieved some signature $\Sigma'$ earlier from its challenger. Under our assumptions so far, both of these are valid signatures for $(m^*,\Ring^*)$. Now if $\Sigma^* = \Sigma'$ then $\Adv_\textsc{euf}$ cannot use $\Sigma^*$ as its forgery, since it has already seen it as a query response. However, the probability that $\Sigma^* = \Sigma'$ is at least $\eta_\RS$ from our earlier arguments (recall that $\Adv_\textsc{bu}$ never sees $\Sigma'$) and so we have that in this case the forgery $(m^*,\Ring^*,\Sigma^*)$ can still be used by $\Adv_\textsc{euf}$ with probability $1-\eta_\RS$. It is easy to see that overall, if $\Adv_\textsc{bu}$ succeeds with probability $\nu$, then $\Adv_\textsc{euf}$ still succeeds with probability at least $(1-\eta_\RS)\nu$. This is still non-negligible ($\eta_\RS$ is at most a constant), and so our claim follows.  
\fi
\end{proof}





==> sections/pq-anonymity.tex <==
%!TEX root=../main.tex

\subsubsection{Post-Quantum Anonymity}
\label{sec:prove:pq:anonymity}
We establish the post-quantum anonymity by proving the following lemma.
\begin{lemma}
\label{lem:ring-sig:pq:anonymity}
    Assume $\algo{LE}$ satisfies the lossiness (\Cref{def:LE:property:lossyness}) described in \Cref{def:special-LE}, $\algo{SPB}$ is index hiding, and $\algo{ZAP}$ is statistically witness indistinguishable. Then, \Cref{constr:pq:ring-sig} satisfies the post-quantum anonymity described in \Cref{def:pq:anonymity}.
\end{lemma}

\xiao{give a sketch of this proof, and move the full proof to the appendix.}

Let $\Adv$ be a QPT adversary participating in \Cref{expr:pq:anonymity}. Recall that the classical identities specified by $\Adv$ is $(i_0, i_1)$ and the quantum query is $\sum_{\Ring, m, t} \psi_{\Ring, m, t} \ket{\Ring, m, t}$. We will show a sequence of hybrids where the challenger switches from signing using $i_0$ to signing using $i_1$. It is easy to see that the scheme is post-quantum anonymous if $\Adv$ cannot tell the difference between each pair of adjacent hybrids.

\para{Hybrid $H_0$:} This hybrid simply runs the anonymity game with $b=0$. That is, $\Adv$'s query is answered as follows:
$$\sum_{\Ring, m, t}\psi_{\Ring, m, t} \ket{ \Ring, m, t} \mapsto \sum_{\Ring, m, t}\psi_{\Ring, m, t} \ket{\Ring, m, t\xor f(\Ring, m)},$$
where
$f(\Ring, m) \coloneqq
\begin{cases}
\RS.\Sign(\SK_{i_0}, \Ring, m;r) & \text{if}~\VK_{i_0}, \VK_{i_1} \in R \\
\bot & \text{otherwise}
\end{cases}
$. We remark that $f(\Ring,m)$ is performed quantumly for each $(\Ring, m)$ pair in the superposition. We say that $\Adv$ {\em wins} if it outputs $b' = b$ $(= 0)$.

It is worth noting that although $\RS.\Sign$ is a randomized algorithm, it uses only a single random tape $r$ for all the $(\Ring, m)$ pairs in the superposition (See \Cref{rmk:single-randomness}). In \Cref{constr:pq:ring-sig}, this means that the $(hk_1, shk_1, hk_2, shk_2, \PI_1, \PI_2, \PI_3)$ values are only sampled once (i.e., they remain the same for all the $(\Ring, m)$ pairs in the superposition).


\para{Hybrid $H_1$:} Recall that in $H_0$, the 2nd (classical) \SPB key pair $(hk_2, shk_2)$ is generated using identity $i_0$. In this hybrid, we generate them using identity $i_1$: 
$$(hk_2, shk_2) \gets \SPB.\Gen(1^\secpar, M, i_1).$$
Everything else in $H_1$ remains identical to $H_0$.

\subpara{$H_0 \cind H_1$:} This follows immediately from the index hiding property (against QPT adversaries) of \SPB defined in \Cref{def:SPB-hash}. Note that $\Adv$'s quantum access to the signing algorithm does not affect this proof at all. Because, as mentioned above in $H_0$, the \SPB key generation happens (classically) only once for all the rings and messages in superposition.



% \para{Hybrid $H_2$:} In this hybrid, we switch the encryption keys for the signature to lossy ones, as opposed to injective ones as before. Namely, for all $i \in [Q]$, $pk_i$ is sampled as $pk_i \gets \KSam^\ls(1^\secpar)$. The corresponding randomness for key generation is now obtained as $r_i = \Set{\RndExt(pk_i)}_{i \in [Q]}$.   

% \subpara{$H_1 \cind H_2$:} We reduce this to the oblivious indistiguishability of lossy and injective keys, as defined in \Cref{def:LE:property:oblivious-mode} of \Cref{def:special-LE}. The reduction simply receives $Q$ pairs of keys and random strings $(pk_i,r_i)_{i \in [Q]}$, and proceeds to use these just as in $H_1$. Namely, it uses the provided $pk_i$s as public keys, and provides the randomness $r_i$ whenever the adversary corrupts user $i$ (note here that the procedure $\RndExt$ is crucial to the reduction in the case where $pk_i$s are lossy). Thus this corresponds to running $H_1$ whenever $pk_i$s are generated using $\KSam$ (and randomness $r_i$), and in turn this corresponds to running $H_2$ whenever $pk_i$s are generated using $\KSam^\ls$ (and `randomness' $\RndExt(pk_i)$). If the adversary has distinguishable outputs in these hybrids, the reduction can tell apart the two possible distributions of $(pk_i,r_i)_{i \in [Q]}$, which violates \Cref{def:LE:property:oblivious-mode}. We note in passing that while this property only guarantees computational indistinguishability (w.r.t classical attackers), this suffices for our argument here: the change between these hybrids occurs in the key generation phase of the challenge, and thus are already in place by the time the adversary makes any (quantum) signing queries. There is thus no question of the adversary having quantum access to these parameters at the time of generation.   



\para{Hybrid $H_2$:} In this hybrid, for each signing query from $\Adv$, instead of sampling $r_{c_2} \gets \PI_2(\Ring\|m)$, we instead compute $r_{c_2}$ as the output of a {\em random} function $r_{c_2} \gets P_2(\Ring\|m)$. In effect, $r_{c_2}$ is now randomly sampled for each $(\Ring, m)$ pairs.  

\subpara{$H_1 \idind H_2$:} 
% The only thing that changes here is the generation of $r_{c_2}$ for each signature in the superposition queried by \Adv. Consider oracles that provide quantum access to $r_{c_2} \gets \PI_2(\Ring\|m)$ and $r_{c_2} \gets P_2(\Ring\|m)$ respectively. We can consider an efficient algorithm $B$ that runs against \Adv and implements $H_2$ (resp. $H_3$) given access to the first (resp. the second) oracle. However, 
This follows from \Cref{lemma:2qwise}. 
% Thus the outputs in both these hybrids are distributed identically. 

\para{Hybrid $H_3$:} Here we switch $c_2$ from an encryption of a zero string to $c_2 \gets \algo{LE.Enc}(pk_{i_1},(\sigma',vk_{i_1});r_{c_2})$, where $\sigma' \gets \Sig.\Sign(sk_{i_1}, m)$. In this hybrid, it is worth noting that the previous ``dummy block'' $(c_2, hk_2, h_2)$ becomes a valid one, where $c_2$ encrypting a valid signature for $m$ using identity $i_1$, $hk_2$ is a $\SPB$ hashing key binding identity $i_1$, and $h_2$ is a hash of $\Ring$ using $hk_2$.

\subpara{$H_2 \sind H_3$:} In both $H_2$ and $H_3$, $r_{c_2}$ is sampled (effectively) uniformly at random for each $(\Ring, m)$ pair in the superposition in each signing query. Consider an oracle $\mathcal{O}$ that takes $(\Ring, m)$ as input and returns $(c_1,c_2,\pi)$ just as in $H_2$, and an analogous oracle $\mathcal{O}'$ that takes the same input and returns $(c_1,c_2,\pi)$ computed just as in $H_3$. Note that the only difference between the outputs of $\mathcal{O}$ and $\mathcal{O}'$ is in $c_2$, which encrypts $0^{|\sigma|+|vk|}$ in $H_2$ and $\sigma',vk_{i_1}$ in $H_3$. Recall that $pk_{i_1}$ is produced using $\LE.\KSam^\ls$ and therefore by lossiness (\Cref{def:LE:property:lossyness}), we have that the distributions of $c_2$ in $H_2$ and $H_3$ are statistically indistinguishable, implying that the outputs of $\mathcal{O}$ and $\mathcal{O}'$ are statistically close for every input $(m,\Ring)$, say less than distance $\Delta$ (which is negligible in \secpar). Then, by \Cref{lemma:oracleindist}, the probability that $\Adv$ distinguishes these two oracles even with $q$ quantum queries is at most $\sqrt{8C_0q^3\Delta}$, which is negligible since $\Delta$ is negligible and $q$ is polynomial. Similarity of these hybrids is immediate. 



\para{Hybrid $H_4$:} In this hybrid, we switch back to using the pairwise independent hash function $\PI_2$ to compute $r_{c_2}$, instead of using a truly random function. Effectively we are undoing the change made in $H_2$. 

\subpara{$H_3 \idind H_4$:} This again follows from \Cref{lemma:2qwise}.



\para{Hybrid $H_5$:} Here, we compute $r_\pi$ as the output of a {\em random} function $r_\pi \gets P_3(\Ring\|m)$, instead of being computed using $\PI_3$ as before. In effect, $r_\pi$ is now uniformly random. 

\subpara{$H_4 \idind H_5$:} This again follows from \Cref{lemma:2qwise}.  


\para{Hybrid $H_6$:} As mentioned in $H_3$, the ``block'' $(c_2, hk_2, h_2)$ is valid. Recall that in previous hybrids, $\ZAP$ uses the witness $w$ corresponding to the block $(c_1, hk_1, h_1)$. In this hybrid, we switch the witness used by $\ZAP$ from $w$ to $w'=(vk_{i_1},pk_{i_1},i_1,\tau_2, \sigma', r_{c_2})$ (i.e., the witness corresponding to the $(c_2, hk_2, h_2)$ block). 
% \xiao{$w=(vk_{i_0}, pk_{i_0}, i_0, \tau_1,\sigma,r_{c_1})$}

\subpara{$H_5 \sind H_6$:} In both $H_5$ and $H_6$, $r_\pi$ is sampled (effectively) uniformly at random for each $(\Ring, m)$ pairs in the superposition for each query. 
% and all other randomness used to compute the reduction is derived deterministically from the message and the ring. 
Consider an oracle $\mathcal{O}$ that takes $(\Ring,m)$ as input and returns $(c_1,c_2,\pi)$ just as in $H_5$, and an analogous oracle $\mathcal{O}'$ that takes the same input and returns $(c_1,c_2,\pi)$ computed just as in $H_6$. Note that the only difference between the outputs of $\mathcal{O}$ and $\mathcal{O}'$ is in $\pi$, which is generated using $w$ in $H_5$ and using $w'$ in $H_6$. Since both $w$ and $w'$ are valid witnesses, by the statistical witness indistinguishability of $\algo{ZAP}$, we have that the distributions of $\pi$ in $H_5$ and $H_6$ are statistically indistinguishable for every $(\Ring, m)$ pair (aka the input to the $\mathcal{O}$ or $\mathcal{O}'$). In other words, the outputs of $\mathcal{O}$ and $\mathcal{O}'$ are statistically close for every input $(m,\Ring)$, say less than distance $\Delta$ (which is negligible in \secpar). Then, the statistical indistinguishability follows from \Cref{lemma:oracleindist}. 


\para{Hybrid $H_7$:} In this hybrid, we switch back to using the pairwise independent hash function $\PI_3$ to compute $r_\pi$, instead of using a truly random function. Effectively we are undoing the change made in $H_5$.

\subpara{$H_6 \idind H_7$:} This again follows from \Cref{lemma:2qwise}.


\para{Hybrid $H_8$:} In this hybrid, instead of sampling $r_{c_1} \gets \PI_1(\Ring\|m)$, we instead compute $r_{c_1}$ as the output of a {\em random} function $r_{c_1} \gets P_1(\Ring\|m)$. In effect, $r_{c_1}$ is now randomly sampled.

\subpara{$H_7 \idind H_8$:} This again follows from \Cref{lemma:2qwise}.




\para{Hybrid $H_{9}$:} In this hybrid, we now switch $c_1$ from an encryption of $(\sigma, vk_{i_0})$ to one of $(\sigma', vk_{i_1})$.

\subpara{$H_8 \sind H_{9}$:} This follows from the same argument for $H_2\sind H_3$. 



\para{Hybrid $H_{10}$:} In this hybrid, we switch back to using the pairwise independent hash function $\PI_1$ to compute $r_{c_1}$, instead of using a truly random function. Effectively we are undoing the change made in $H_8$.

\subpara{$H_{9} \idind H_{10}$:} This again follows from \Cref{lemma:2qwise}.  


\para{Hybrid $H_{11}$:} In this hybrid, the \SPB key pair $(hk_1, shk_1)$ is now generated using identity $i_1$, instead of $i_0$. Namely, we compute  $(hk_1, shk_1) \gets \SPB.\Gen(1^\secpar, M, i_1)$.

\subpara{$H_{10} \cind H_{11}$:} This follows from the same argument for $H_0 \cind H_1$.



\para{Hybrid $H_{12}$:} In this hybrid, we switch to computing $r_\pi$ as the output of a {\em random} function $r_\pi \gets P_3(\Ring\|m)$, instead of being computed using $\PI_3$.  

\subpara{$H_{11} \idind H_{12}$:} This again follows from \Cref{lemma:2qwise}.  



\para{Hybrid $H_{13}$:}In this hybrid, we again switch the witness used to generate $\pi$, from $w'$ to $w''=(vk_{i_1},pk_{i_1},i_1,\tau_1,\sigma',r_{c_1})$.
 
\subpara{$H_{12} \sind H_{13}$:} This follows from the same argument for $H_5 \sind H_6$. 


\para{Hybrid $H_{14}$:} In this hybrid, we switch back to using the pairwise independent hash function $\PI_3$ to compute $r_\pi$, instead of using a truly random function. 

\subpara{$H_{13} \idind H_{14}$:} This again follows from \Cref{lemma:2qwise}.  



\para{Hybrid $H_{15}$:} Here, we switch to computing $r_{c_2}$ as the output of a {\em random} function $r_{c_2} \gets P_2(\Ring\|m)$.

\subpara{$H_{14} \idind H_{15}$:}  This again follows from \Cref{lemma:2qwise}.  

\para{Hybrid $H_{16}$:} In this hybrid, we switch $c_2$ to an encryption of zeroes, namely $c_2 \gets \LE.\Enc(pk, 0^{|\sigma|+|vk|}; r_{c_2})$, instead of an encryption of $(\sigma',vk_{i_1})$.

\subpara{$H_{15} \sind H_{16}$:} This argument is identical to that for simlarity between $H_2\sind H_3$.



\para{Hybrid $H_{17}$:} In this hybrid, we switch back to using the pairwise independent hash function $\PI_2$ to compute $r_{c_2}$, instead of using a truly random function. 

\subpara{$H_{16} \idind H_{17}$:} This again follows from \Cref{lemma:2qwise}.  

% \para{Hybrid $H_{18}$:} In this hybrid, we switch the encryption keys for the ring signature back to injective ones. Namely, for all $i \in [Q]$, the challenger samples $r_i$ uniformly and computes $pk_i \gets \KSam(1^\secpar)$

% \subpara{$H_{17} \cind H_{18}$:} The argument for this is essentially the same as that showing similarity between $H_1$ and $H_2$.
\vspace{1em}

Observe that $H_{17}$ corresponds to sign using identity $i_1$ in \Cref{expr:pq:anonymity}. This finishes the proof of \Cref{lem:ring-sig:pq:anonymity}.

% % Xiao's outline for anonymity
% \para{Hybrid $H_2$:} \xiao{switch to lossy $pk$ of $\LE$. That is, for all $i \in [Q]$, $pk_i$ is sampled as $pk_i \gets \KSam^\ls(1^\secpar)$.}

% \subpara{$H_1 \cind H_2$:} \xiao{due to the Oblivious IND of the lossy and injective mode (see how I formalize it in \Cref{def:LE:property:oblivious-mode} of \Cref{def:special-LE}). Explain that we do need \Cref{def:LE:property:oblivious-mode} as we are in the fully key exposure setting (we also need to fake the randomness for $\Adv$ by giving $\Set{\RndExt(pk_i)}_{i \in [Q]}$). It seems our crypto paper missed this argument.}

% \xiao{
% Also say that $\Adv$'s quantum access to the signing algorithm does not affect this proof, because the $pk_i$'s (contained in $\VK_i$'s) are sampled classically by the challenger before $\Adv$ makes any quantum {\bf sign} queries happens.}

% \para{Hybrid $H_3$:} \xiao{switch $c_2$ to a ciphertext of $\sigma' \gets \Sig.\Sign(sk_{i_1}, m)$. (This is the $H_2$ (on Page 28) in our crypto paper).} 

% \subpara{$H_2 \sind H_3$:} \xiao{Since we are in the lossy mode of $\LE$, each ciphertexts of $\LE$ differs statistically negligibly. So, this statistical indistinguishability follows from \Cref{lemma:oracleindist}. (Give a kind-of detailed explanation.)}

% \para{Hybrid $H_4$:} \xiao{Switch the witness used by our ZAP.(This is the $H_3$ (on Page 28) in our crypto paper).}

% \subpara{$H_3 \sind H_4$:} \xiao{Note that our ZAP is {\em statistically} WI. So, this statistical indistinguishability follows again from \Cref{lemma:oracleindist}. (Give a kind-of detailed explanation).}

% \para{Hybrid $H_5$:} \xiao{Switch $c_1$ to an encryption of $\sigma' \gets \Sig.\Sign(sk_{i_1}, m)$). (Recall that $c_1$ was a ciphertext of $\sigma' \gets \Sig.\Sign(sk_{i_0}, m)$.)}

% \subpara{$H_4 \sind H_5$:} \xiao{Again, we are in the lossy mode. So, this follows from \Cref{lemma:oracleindist}.}

% \para{Hybrid $H_6$:} \xiao{sample the 1st SPB key pair using identity $i_1$. That is, $$(hk_1, shk_1) \gets \SPB.\Gen(1^\secpar, N, i_1).$$}

% \subpara{$H_5 \cind H_6$:} \xiao{follow the same argument as for $H_0 \sind H_1$.}


% \para{Hybrid $H_7$:} \xiao{switch ZAP witness back to the first block, as now it is a valid ciphertext for signatures using $i_1$.}

% \subpara{$H_6 \sind H_7$:} \xiao{same as $H_3 \sind H_4$.}


% \para{Hybrid $H_8$:} \xiao{change $c_2$ back to $\LE.\Enc(pk, 0^{|\sigma|+|vk|}; r_{c_2})$.}

% \subpara{$H_7 \sind H_8$:} 
% \xiao{Notice that we are still in the lossy mode. So, same argument as for $H_2 \sind H_3$.}

% \para{Hybrid $H_9$:} \xiao{change to injective mode. That is, for all $i\in [Q]$, $pk_i$ is sampled as $pk_i \gets \KSam(1^\secpar)$.}

% \subpara{$H_8 \sind H_9$:} 
% \xiao{same as for $H_1 \cind H_2$.}

 

==> sections/pq-unforgeability.tex <==
%!TEX root=../main.tex
\subsubsection{Post-Quantum Blind-Unforgeability}
\label{sec:prove:pq:blind-unforgeability}

In this section, we prove the following lemma.
\begin{lemma}
\label{lem:ring-sig:pq:blind-unforgeability}
    Assume $\Sig$ is blind-unforgeable as per \Cref{def:classical-BU-sig}, $\algo{LE}$ satisfies the almost-unique secret key property (\Cref{item:def:LE:computationally-unique-sk}), $\algo{SPB}$ is somewhere perfectly binding, and $\algo{ZAP}$ has the selective non-witness adaptive-statement soundness (\Cref{item:def:zap:soundness}). Then, \Cref{constr:pq:ring-sig} is blind-unforgeable as  per \Cref{def:pq:blind-unforgeability}.
\end{lemma}

Consider a QPT adversary $\Adv_\RS$ participating in \Cref{expr:pq:blind-unforgeability}. We proceed with a sequence of hybrids to set up our reduction to the blind-unforgeability of \algo{Sig}.
    
\para{Hybrid $H_0$:} This is just the post-quantum blind-sunforgeability game (\Cref{expr:pq:blind-unforgeability}) for our construction. In particular, for all $i\in [Q]$, the encryption key $pk_i$ is generated as $pk_i\gets \LE.\KSam^\ls(1^\secpar)$.   

\para{Hybrid $H_1$:} In this experiment, the only difference is that, the challenger first picks a uniformly random secret key for $\LE$ as $sk_\LE \pick \mathcal{SK}_\secpar$, and then generates the corresponding public keys for the adversary using this, namely $pk_i \gets \algo{LE.GenWithSK}(sk_{\LE})$ for all $i \in [Q]$. The challenger now stores $sk_{\LE}$.

\subpara{$H_0 \cind H_1$:} This follows immediately from the IND of $\GenWithSK$/$\KSam^\ls$ property (\Cref{def:LE:property:IND:GenWithSK-KSam}) of $\LE$ as specified in \Cref{def:special-LE}. It is worth noting that $\Adv_\RS$'s quantum access to the signing algorithm does not affect this proof at all. Because the $pk_i$'s (contained in $\VK_i$'s) are sampled classically by the challenger before $\Adv_\RS$ makes any quantum {\sf sign} queries.

\para{Reduction to the BU of $\Sig$.} We proceed to show that post-quantum blind-unforgeability holds in $H_1$. Consider the adversary's forgery attempt 
$$\big(\algo{R}^*, m^*, \Sigma^* = (c_1^*, hk_1^*,c_2^*,hk_2^*,\pi^*)\big)~\text{satisfying}~(\Ring^*, m^*) \in B^\RS_\epsilon.$$ 
Let $x_1^*$ be the statement corresponding to $\Sigma^*$: $x_1^* \coloneqq (m^*,c_1^*,c_2^*,hk_1^*,hk_2^*,h_1^*,h_2^*)$, where $h_1^* = \algo{SPB.Hash}(hk_1^*,\mathsf{R^*})$ and $h_2^* = \algo{SPB.Hash}(hk_2^*,\mathsf{R^*})$. Let $x^*_2 \coloneqq \Ring^*$ and $x^* \coloneqq (x^*_1, x^*_2)$. Let $\algo{VK}_1^*$ = ($vk_1^*,pk_1^*,\rho_1^*$) be the lexicographically smallest verification key in $\algo{R}^*$.  

Observe that for the $x^*$ defined above, one of the following two cases must happen: $x^* \in \tilde{L}$ or $x^* \notin \tilde{L}$. (Recall that $\tilde{L}$ is the super-complement of $L$ defined in \Cref{eq:def:language:L-tilde}.) In the following, we show two claims. \Cref{lemma:unfroge:inltilde} says that it cannot be the case that $x^* \in \tilde{L}$, unless the $\ZAP$ verification rejects (thus, the forgery is invalid). \Cref{lemma:unforge:sig} says that $x^* \notin \tilde{L}$ cannot happen either. Therefore, \Cref{lemma:unfroge:inltilde,lemma:unforge:sig} together show that any QPT adversary has negligible chance of winning the blind-unforgeability game for $\RS$ in $H_1$. Note that winning the post-quantum blind-unforgeability game for $\RS$ is an event that can be efficiently tested. Thus, by $H_0 \cind H_1$, no QPT adversaries can win the post-quantum blind-unforgeability game for $\RS$ in hybrid $H_0$. This eventually finishes the proof of \Cref{lem:ring-sig:pq:blind-unforgeability}.

Now, the only thing left is to state and prove \Cref{lemma:unfroge:inltilde,lemma:unforge:sig}, which is done in the following. 

    

 \begin{MyClaim}
    	\label{lemma:unfroge:inltilde}
    	In $H_1$, assume that $\algo{ZAP}$ satisfies selective non-witness adaptive statement soundness (\Cref{item:def:zap:soundness}). %, and $\LE$ has injective key generation \xiao{check this injectivity.}. 
    	Then, the following holds:
    	$$\Pr[x^* \in \widetilde{L}  ~\wedge~ \algo{\algo{ZAP}.Verify}(\rho_1^*,x^*,\pi^*)=1] = \negl(\lambda).$$
    \end{MyClaim}   
\begin{proof}
% \xiao{This lemma is identical to \cite[Lemma 5.5]{C:CGHKLMPS21}. May go to the appendix.}
First, notice that by definition, the $\Ring^*$ in $\Adv_\RS$'s forgery contains only $\VK$'s from the set $\mathcal{VK} = \Set{\VK_j}_{j\in [Q]}$ generated by the challenger. Therefore, it suffices to show that for each $j \in [Q]$, 
\begin{equation}\label{eq:lemma:unfroge:inltilde:real-goal}
\Pr[x^*  \in \widetilde{L} ~\wedge~ \algo{ZAP.Verify}(\rho_j,x^*,\pi^*)=1] = \negl(\lambda),
\end{equation}
where $\rho_j$ denotes the first-round message of \ZAP corresponding to the $j$-th verification key $\algo{VK}_j$ generated in the game.

Let $\Adv_\RS$ be an adversary attempting to output a forgery such that $x^* \in \widetilde{L}$ {\em and} $\algo{ZAP}.\Verify(\rho_j,x^*,\pi^*) =1$. We build an adversary $\Adv_\ZAP$ against the selective non-witness adaptive-statement soundness of $\algo{ZAP}$ for $(L, \widetilde{L})$ (defined in \Cref{eq:def:language:L,eq:def:language:L-tilde} respectively). % with the fixed non-witness $\widetilde{w} = sk_{\LE}$.
The algorithm $\Adv_\ZAP$ proceeds as follows: 
    	\begin{itemize}
    		\item On input the first \algo{ZAP} message $\widehat{\rho}$, it sets $\rho_{j} = \widehat{\rho}$ and then proceeds exactly as $H_1$. 
    		\item Upon receiving the forgery attempt $(\Ring^*, m^*, \Sigma^*)$ from $\Adv$, it constructs the corresponding $x^*$ and $\pi^*$, and outputs $(x^*,\pi^*)$.
    	\end{itemize} 

We remark that $H_1$ is quantum. So, $\Adv_\ZAP$ needs to be a quantum machine to simulate $H_1$ for $\Adv_\RS$. This is fine since we assume that the soundness (\Cref{item:def:zap:soundness}) of ZAP in \Cref{def:generalizedzap-interface} holds against QPT adversaries. 

To finish the proof, notice that $x^* \in \widetilde{L}$ means that there exists a non-witness $\tilde{w}^*$ such that $(x^*, \tilde{w}^*) \in \tilde{R}$. Therefore, if \Cref{eq:lemma:unfroge:inltilde:real-goal} does not hold, $(\rho_j, x^*, \pi^*)$ will break the soundness (\Cref{item:def:zap:soundness}) w.r.t.\ the non-witness $\tilde{w}$.
% -- Sina's argument using an explicit $\tilde{w} = sk_\LE$ is not necessary. We only need the {\em existence} of $\tilde{w}$, which is guaranteed by the assumption that $x^* \in \tilde{L}$. 
% then $(x^*, sk_{\LE}) \in \widetilde{R}$ (except with negligible probability). This is because, if $x^* \in \widetilde{L}$, then, by definition of $\widetilde{L}$ (in particular, the $R_4$ in \Cref{def:relation:R4}), there exists a non-witness $\widetilde{w}^*$ such that, 
%     	\[\forall (vk_i^*, pk_i^*, \rho_i^*) \in \algo{R}^*:  \LE.\Valid(pk_i^*,\widetilde{w}^*)=1; \]
% and since $\LE$ has \xiao{injective key generation}, it follows that except with negligible probability, $\widetilde{w}^* =  sk_{\LE}$ $(= \tilde{w})$. Therefore, if \Cref{eq:lemma:unfroge:inltilde:real-goal} does not hold, $(\rho_j, x^*, \pi^*)$ will break the soundness (\Cref{item:def:zap:soundness}) w.r.t.\ the non-witness $\tilde{w} = sk_\LE$.
\end{proof}

\begin{MyClaim}
	\label{lemma:unforge:sig}
	In $H_1$, assume that $\algo{Sig}$ satisfies the blind-unforgeability as per \Cref{def:classical-BU-sig}, $\LE.\GenWithSK$ has the almost-unique secret key property defined in \Cref{item:def:LE:computationally-unique-sk}, 
	and $\algo{SPB}$ is somewhere perfectly binding. Then,
	$\Pr\big[x^* \not \in \widetilde{L}\big] = \negl(\lambda)$.
\end{MyClaim}
\begin{proof}
Let $\Adv_\RS$ be a QPT adversary attempting to output a forgery w.r.t.\ our $\RS$ scheme such that $x^* \not \in \widetilde{L}$. We build an algorithm $\Adv_\Sig$ against the  blind-unforgeability of $\algo{Sig}$. The algorithm $\Adv_\Sig$ (playing the blind-unforgeability game \Cref{expr:BU:ordinary-signature} for $\Sig$) proceeds as follows:

\begin{enumerate}
	\item 
	invoke $\Adv_\RS$ to obtain the $\epsilon$ for the blind-unforgeability game of $\RS$; give this $\epsilon$ to $\Adv_\Sig$'s own challenger for the blind-unforgeability game of $\Sig$;
	
	\item
	receive $\widehat{vk}$ from its own challenger; pick an index $j \pick [Q]$ uniformly at random; set $vk_{j} \coloneqq \widehat{vk}$; then, proceeds as in $H_1$ to prepare the rest of the verification keys and continue the execution with $\Adv_\RS$.
	
	\item \label[Step]{step:unforge:sig:signing-query}
	when $\Adv_\RS$ sends a quantum signing query $(\algo{sign},i, \sum \psi_{\Ring, m, t}\ket{\Ring, m, t})$, if the specified identity $i$ is not equal to $j$, it proceeds as in $H_1$; otherwise, it uses the blind-unforgeability (for $\Sig$) game's signing oracle $\Sig.\Sign$ to obtain a $\Sig$ signature for the $j$-th party and then continues exactly as in $H_1$; (See the paragraph right after the description of $\Adv_\Sig$.)

	\item 
	if $\Adv_\RS$ tries to corrupt the $j$-th party, $\Adv_\Sig$ aborts; (It is worth noting that the identities are classical. So, $\Adv_\RS$'s quantum access to the signing oracle does not affect this step.)

	\item 
	upon receiving the forgery attempt $\Sigma^*$ from $\Adv_\RS$, $\Adv_\Sig$ decrypts $c_1^*$ using $sk_\LE$ to recover $\sigma_1^*$. If  $\algo{Sig.Verify}(vk_j,m^*, \sigma_1^*) \text{ accepts}$, it sets $\widehat{\sigma} := \sigma_1^*$. Otherwise, it decrypts $c_2^*$ with $sk_\LE$ to recover $\sigma_2^*$, and sets $\widehat{\sigma} \coloneqq \sigma_2^*$. It outputs $(m^*,\widehat{\sigma})$. 
\end{enumerate}

We first remark that, up to (inclusively) \Cref{step:unforge:sig:signing-query}, $\Adv_\RS$'s view is identical to that in $H_1$. Recall that in $H_1$, the challenger maintains a blindset $B_\epsilon$ such that any $(\Ring, m) \in B^\RS_\epsilon$ will not be answered (this is inherited from $H_0$, which is exactly \Cref{expr:pq:blind-unforgeability}). In contrast, in the execution of $\Adv_\Sig$ described above, $\Adv_\Sig$ first forwards the $\sum \psi_{\Ring, m, t}\ket{\Ring, m, t}$ part of $\Adv_\RS$'s query to its $\Sig.\Sign$ oracle to obtain 
$$\sum_{\Ring, m, t} \psi_{\Ring, m, t} \ket{\Ring, m, t\xor \Sig.\Sign(sk_j, \Ring\|m)}, \text{ (note that $sk_j = \widehat{sk}$)}$$ and then performs the remaining computation exactly as in $H_1$. Note that the $\Sig$ signing oracle also maintains a blindset $B^\Sig_\epsilon$ for $\Sig$'s message sapce; and importantly, since the ``messages'' singed by $\Sig$ are of the form $\Ring\|m$, $B^\Sig_\epsilon$ is actually generated identically to $B^\RS_\epsilon$---that is, both of them are generated by including each $(\Ring, m)$ pair in with (the same) probability $\epsilon$.

To finish the proof, we show that 
$(\Ring^*\|m^*,\widehat{\sigma})$ is a valid forgery against $\Sig$'s blind-unforgeability game with probability at least $\frac{1}{Q}\big(\Pr\big[x^* \not \in \widetilde{L}\big]- \negl(\lambda)\big)$.

Recall that we are focusing on the case $x^* \notin \tilde{L}$, where $\tilde{L}$ is defined in \Cref{eq:def:language:L-tilde}; without loss of generality, assume that $(m^*, c_1^*, hk_1^*, h_1^*, \algo{R^*}) \not \in \widehat{L}$. Then, observe that due to the way $H_1$ generates the public keys and also the definition of $h_1^*$, we know that
    	\begin{equation}\label[Expression]{eq:unforge:sig:proof:L4}
    	\big((m^*,c_1^*,hk_1^*,h_1^*,\algo{R^*}), sk_\LE\big) \in R_4 ~~\text{(recall that $R_4$ is defined in \Cref{def:relation:R4})}.
    	\end{equation}
Since we assume that $(m^*,c_1^*,hk_1^*,h_1^*,\algo{R^*}) \notin \widehat{L}$, \Cref{eq:unforge:sig:proof:L4} and the definition of $\widehat{L}$ imply the existence of a string $\widetilde{w}$ such that
\begin{equation}\label[Expression]{eq:unforge:sig:proof:L5}
\big((m^*,c_1^*,hk_1^*,h_1^*,\algo{R^*}),\widetilde{w}\big)  \in R_5 ~~\text{(recall that $R_5$ is defined in \Cref{def:relation:R5})}.
\end{equation}
By the almost-unique secret key property of $\LE.\GenWithSK$ (\Cref{item:def:LE:computationally-unique-sk}), it follows that $\widetilde{w} = sk_\LE$ (except with negligible probability). Consequently, the following hold:
\begin{enumerate}
	\item 
	by our assumption, $(\Ring^*, m^*) \in B^\RS_\secpar$; this also implies $(\Ring^*, m^*) \in B^\Sig_\secpar$ because $B^\Sig_\epsilon = B^\RS_\epsilon$ as argued earlier;

\item 
by \Cref{eq:unforge:sig:proof:L4} and the somewhere perfectly binding property of \algo{SPB}, there exists $\algo{VK^*} = (vk^*,pk^*,\rho^*)$ such that 
$$\algo{VK}^* \in \algo{R^*} ~~\text{and}~~ \LE.\Valid(pk^*, sk_\LE) = 1;$$

\item
by \Cref{eq:unforge:sig:proof:L5}, $\LE.\Dec\big(\tilde{w} ~(= sk_\LE),c_1^*\big) = (\sigma^*,vk^*)$ for some $\sigma^*$ and $vk^*$ and $\algo{Sig.Verify}(vk^*, \Ring^*\|m^*,\sigma^*)=1$.
\end{enumerate}
The above means that the $\Adv_\Sig$ uses a verification key $\algo{VK^*} \in \mathsf{R^*}$ and that $c_1^*$ encrypts (among other things) a signature $\sigma^*$ that is valid for the forgery message $\Ring^*\|m^*$ w.r.t. key $vk^*$ for the blind-unforgeability game of $\Sig$. Moreover, $\Adv_\Sig$ can extract this forgery message efficiently by decrypting $c^*$ using $sk_\LE$!

Finally, observe that index $j$ is sampled uniformly. 
Therefore, we have that $(\widehat{vk} =)$ $vk_j = vk^*$ with probability $1/Q$.
\end{proof}

==> sections/ring-sig-construction.tex <==
%!TEX root=../main.tex


To conclude, we present the complete definition of post-quantum secure ring signatures as follows.
\begin{definition}[Post-Quantum Secure Ring Signatures]
\label{def:pq:ring-signatures}
A post-quantum secure ring signature scheme $\RS$ is described by a triple of PPT algorithms $(\Gen,\Sign,\Verify)$ that share the same syntax as in \Cref{def:classical:ring-signature}. Moreover, they also satisfy the {\em completeness} requirement in \Cref{def:classical:ring-signature}, the {\em post-quantum anonymity} in \Cref{def:pq:anonymity}, and the {\em post-quantum blind-unforgeability} as in \Cref{def:pq:blind-unforgeability}.
\end{definition}

\subsection{Building Blocks}
\subsubsection{Somewhere Perfect Binding Hash}

As in \cite{EC:BDHKS19,C:CGHKLMPS21}, we will only define and employ somewhere perfectly binding hash functions {\em with private local openings}. We present the definition from \cite{C:CGHKLMPS21} with following modification. In \cite{C:CGHKLMPS21} (inherited from \cite{ITCS:HubWic15,EC:BDHKS19}), the $\SPB.\Gen$ algorithm needs a parameter $n$ specifying the size of the database that will be hashed later. Due to a technical reason in our application, we need to make $\SPB.\Gen$ depend only on the {\em upper bound} of supported databases' size. That is, running $\SPB.\Gen$ on an integer $M$ will yield a key that can be used to hash any database of size $\le M$. Fortunately, existing constructions achieve this property by setting $M$ to be super-polynomial on $\secpar$ and padding any database of size $\le M$ with some special symbol (e.g., ``$\bot$'') before hashing. This will not blow up the running time of $\algo{SPB.Hash}$ because the subtree with only ``$\bot$'' leaves is dummy, thus $\algo{SPB.Hash}$ does not really to compute it. 

Also, the standard efficiency property of SPB usually requires that the $\algo{SPB.Open}$ and $\algo{SPB.Verify}$ algorithms run in logarithmic time on the actual database size. In contrast, our definition relaxes this to be logarithmic on the upper bound parameter $M$. This already suffices for our application (see \Cref{rmk:SPB:setting-M}).

\begin{remark}[On efficiency]\label{rmk:SPB:setting-M}
In applications (e.g., our \Cref{constr:pq:ring-sig}), one can set, say, $M = 2^{\log^2\secpar}$ such that the SPB scheme can be used to hash any polynomial-size database while still achieving compactness---According to \Cref{item:def:SPB:efficiency} below, if $M = 2^{\log^2\secpar}$, then the efficiency will be $\log(M)\poly(\secpar)=\log^2(\secpar) \poly(\secpar)$, which is effectively independent of the actual size of the database.
\end{remark}

The definition is given as follows. \cite{EC:BDHKS19} builds such a scheme assuming quantum hardness of LWE. 

\begin{definition}[SPB Hash \cite{C:CGHKLMPS21}]\label{def:SPB-hash}
    A {\em somewhere perfectly binding (SPB) hash} scheme with private local openings consists of a tuple of probabilistic polynomial time algorithms $(\algo{Gen,Hash,Open,Verify})$ with the following syntax: 
    
    \begin{itemize}
        
        \item {$\algo{Gen}(1^\lambda, M, \mathsf{ind})$} takes as input an integer $M \le 2^\secpar$ indicating the upper bound of the database size and an index $\mathsf{ind}$; it outputs a key pair $(hk,shk)$. 
        
        \item {$\algo{Hash(hk,db)}$,} given a hash key $hk$ and database \algo{db} as input, outputs a hash value $h$. 
        
        \item {$\algo{Open}(hk,shk,\algo{db,ind})$,} given a hash key $hk$, secret key $shk$, database \algo{db} and index \algo{ind} as input, outputs a witness $\tau$. 
        
        \item {$\algo{Verify}(hk,h,\mathsf{ind},x,\tau)$,} given as input a hash key $hk$, a hash value $h$, an index \algo{ind}, a value $x$ and a witness $\tau$, outputs either 1 (accepting) or 0 (rejecting).
        
    \end{itemize}
    
    To maintain clarity, we will not explicitly specify the block size of databases as input to $\algo{Gen}$, but assume that this is clear from the specific usage and hardwired into the algorithm. Also, for any index $\algo{ind}$ greater than the actual size of a database $\algo{db}$, we use a special symbol ``$\bot$'' to denote the value $\algo{db_{ind}}$. The SPB scheme should satisfy the following properties: 
    
    \begin{enumerate}
        \item {\bf Correctness:} for any $\lambda \in \Naturals$, any $M\le 2^\secpar$, any database \algo{db} of size $\le M$, and any index $\algo{ind} \in [M]$, we have, 
        $$
        \Pr[
            \begin{array}{l}
            (hk,shk) \gets \algo{Gen}(1^\lambda, M,\algo{ind});\\
             h \gets \algo{Hash}(hk,\algo{db}); \\
            \tau \gets  \algo{Open}(hk,shk,\algo{db,ind})
            \end{array}:
            \algo{Verify}(hk,h,\algo{ind}, \algo{db_{ind}},\tau) = 1 
        ] = 1.
        $$
        % \[\Pr[\algo{Verify}(hk,h,\algo{ind,db_{ind}},\tau) \text{ accepts }] = 1,\]
        % where, $(hk,shk) \gets \algo{Gen}(1^\lambda,n,\algo{ind})$, $h \gets \algo{Hash}(hk,\algo{db})$ and $\tau \gets  \algo{Open}(hk,shk,\algo{db,ind})$.
        
        \item \label{item:def:SPB:efficiency}
        {\bf Efficiency:} all hash keys $\algo{hk}$ generated by $ \Gen(1^\secpar, M, \algo{ind})$ and all witnesses $\tau$ generated by $\algo{Open}(hk,shk, \algo{db}, \algo{ind})$ where $|\algo{db}| \le M$ are of size $\log(M)\poly(\lambda)$. Further, for databases of size $\le M$, $\algo{Verify}$ can be computed by a circuit of size $\log(M)\poly(\lambda)$.
        
        \item {\bf Somewhere perfectly binding:} for all $\lambda\in \Naturals$, all $M \le 2^\secpar$, all databases $\algo{db}$ of size $\le M$, all indices $\algo{ind} \in [M]$, all purported hashing keys $hk$, all purported witnesses $\tau$, and all $h$ in the support of $\algo{Hash}(hk,\algo{db})$, it holds that
        $$\algo{Verify}(hk,h,\algo{ind},x,\tau)=1 ~\Rightarrow~ x=\mathsf{db_{ind}}.$$  
        
        \item {\bf Index hiding:} for any $M\le 2^\secpar$ and any $\algo{ind}_0,\algo{ind}_1 \in [M]$,
        \[ \big\{(hk,shk) \gets \algo{Gen}(1^\lambda, M, \algo{ind}_0): hk \big\}_{\secpar \in \Naturals}  \cind  \big\{(hk,shk) \gets \algo{Gen}(1^\lambda,M,\algo{ind}_1) : hk \big\}_{\secpar \in \Naturals} \]
    \end{enumerate}
\end{definition}



\subsubsection{Lossy PKE with Oblivious Key Generation}
\xiao{@Giulio: can you cite the correct work that build a lossy encryption (probably with slight modifications) satisfying \Cref{def:special-LE}?}

\begin{definition}[Special Lossy PKE]\label{def:special-LE}
For any security parameter $\secpar \in \Naturals$, let $\mathcal{M}_\secpar$ denote the message space, and $\mathcal{SK}_\secpar$ denote the {\em PPT-samplable} secret key space.
A special lossy public-key encryption scheme $\algo{LE}$ consists of the following PPT algorithms:
\begin{itemize}
% \item
%  $\Gen(1^\secpar)$ outputs key pairs $(\pk,\sk)$, which we call {\em injective key pairs}.
\item 
 $\algo{GenWithKey}(1^\secpar, \sk)$, on input a secret key $\sk \in \mathcal{SK}_{\lambda}$, outputs $\pk$, which we call {\em injective public key}.

\item
 $\KSam^\ls(1^\secpar)$ outputs key $\pk_\ls$, which we call {\em lossy public key}.
     
\item 
$\algo{Valid}(\pk,\sk)$, on input a public $\pk$ and a secret key $\sk$, outputs either $1$ (accepting) or $0$ (rejecting).

\item
$\RndExt(\pk)$ outputs a $r$ which we call {\em extracted randomness}.


\item 
$\algo{Enc}(\pk, m)$, on input a public key $\pk$, and a message $m \in \mathcal{M}_\secpar$, outputs $\ct$.

\item 
$\algo{Dec}(\sk, \ct)$, on input a secret key $\sk$ and a ciphertext $ct$, outputs $m$.


% \item
% $\KSam(1^\secpar)$ outputs a $\pk$ which we call {\em oblivious injective public key}.
\end{itemize}
These algorithms satisfy the following properties:
\begin{enumerate}
\item \label{item:def:LE:completeness}
{\bf Completeness.} For any $\secpar\in\Naturals$, any $(\pk, \sk)$ s.t.\ $\Valid(\pk, \sk) =1$, and any $m \in \mathcal{M}_\secpar$, it holds that $\Pr[\Dec\big(\sk, \Enc(\pk, m)\big)= m] = 1$.
% classical IND Lossy/Injective mode. Not needed in this paper
% \item
% {\bf Indistinguishability of keys.} \xiao{Once we have the Oblivious IND defined below ($+$ the $\algo{GenWithSK}$ defined later), we may not need this anymore.} Lossy public keys are computationally indistinguishable from injective public keys:
% $$ \big\{ (\pk, \sk) \pick \Gen(1^\secpar,\inj): \pk \big\}_{\secpar\in\Naturals} \cind \big\{ (\pk_\ls, \sk_\ls) \pick \Gen(1^\secpar,\ls): \pk_\ls \big\}_{\secpar\in\Naturals}.$$

\item \label{def:LE:property:lossyness}
{\bf Lossiness of lossy keys.} For any $\pk_\ls$ in the range of $\KSam^\ls(1^\secpar)$ and any $m_0, m_1 \in \mathcal{M}_\secpar$,
$$\big\{ \Enc(\pk_\ls, m_0) \big\}_{\secpar\in\Naturals} \sind \big\{ \Enc(\pk_\ls, m_1) \big\}_{\secpar\in\Naturals}.$$

% \item {\bf Oblivious injective  pulic key generation:} $\KSam$ generates injective public keys with overwhelming probability:
% $$\Pr[\pk \gets \KSam(1^\SecPar): \exists \sk~s.t.~\Valid(\pk,\sk) =1] \ge 1 - \negl(\secpar).$$

% \item \label{def:LE:property:oblivious-mode} 
% {\bf Obliviously IND of \ls/\inj mode:} For any $Q=\poly(\secpar)$, the following two distributions are computationally indistinguishable:
% \begin{itemize}
% \item
% $\forall i\in [Q]$, sample $\pk_i \gets \KSam(1^\secpar; r_i)$, then output $\Set{\pk_i, r_i}_{i\in [Q]}$;
% \item 
% $\forall i\in [Q]$, sample $\pk_i \gets \KSam^\ls(1^\secpar)$, then output $\Set{\pk_i, \algo{RndExt}(\pk_i)}_{i\in [Q]}$.
% \end{itemize}

\item \label{def:LE:property:GenWithSK:completeness}  
{\bf Completeness of $\GenWithSK$:} It holds that
$$\Pr[\sk\pick \mathcal{SK}_\secpar; \pk \gets \GenWithSK(\sk): \Valid(\pk,\sk) =1 ] \ge 1 - \negl(\secpar).$$

\item \label{def:LE:property:IND:GenWithSK-KSam}  
{\bf IND of $\GenWithSK$/$\KSam^\ls$ mode:} For any $Q=\poly(\secpar)$, the following two distributions are computationally indistinguishable:
\begin{itemize}
\item
$\forall i\in [Q]$, sample $\pk_i \gets \KSam^\ls(1^\secpar; r_i)$, then output $\Set{\pk_i, r_i}_{i\in [Q]}$;
\item 
Sample $sk \pick \mathcal{SK}_\secpar$; $\forall i\in [Q]$, sample independently $pk_i \gets \GenWithSK(1^\secpar, sk)$; then, output $\Set{\pk_i, \algo{RndExt}(\pk_i)}_{i\in [Q]}$.
\end{itemize}

\item \label{item:def:LE:computationally-unique-sk}
{\bf Almost-Unique Secret Key:} It holds that
$$
\Pr[
\begin{array}{l}
sk \pick \mathcal{SK}_\secpar;\\
pk \gets \GenWithSK(1^\secpar, sk);
\end{array}: 
\begin{array}{l}
\text{There exists an}~sk'~\text{such that} \\
sk' \ne sk ~\wedge~ \Valid(pk, sk') = 1
 \end{array}
] = \negl(\secpar).
$$
\end{enumerate}
\end{definition}


\subsubsection{Compact ZAPs for Super-Complement Languages}

\para{The Role of ZAPs.} \cite{C:CGHKLMPS21} uses a (special) ZAP for security. It plays a similar role as that of NIZK in the Naor-Yung paradigm \cite{STOC:NaoYun90}: the signing algorithm generates two ciphertexts $(c_1, c_2)$, where $c_1$ encrypts a real signature using the ring and identity specified by the adversary, and $c_2$ encrypts a dummy signature. To establish anonymity, $c_1$ will be switched to an encryption of a signature using another identity. This can be done relying on the WI property of ZAP in a similar manner as in \cite{STOC:NaoYun90}. To establish unforgeability, the hybrid will use the secret key to extract the forgery signature from $c_1$ or $c_2$ output by the adversary, which is used to break the unforgeability of the building-block (ordinary) signature scheme $\Sig$. The soundness of ZAP plays an important role in this argument to ensure that at least one of $(c_1, c_2)$ encrypts a valid signature.

However, ZAPs from \NP are currently not known from LWE. \cite{C:CGHKLMPS21} bypasses this obstacle by constructing a ZAP for $\NP \cap\coNP$ assuming LWE, and shows that it suffices for the ring signature application. Roughly, this is because that if the forgery does not contain a valid signature w.r.t.\ the building-block $\Sig$, then the secret key serves as a non-witness. That is, the hybrid can decrypt both $(c_1, c_2)$ and tell that neither of the plaintexts are a valid $\Sig$ signature. This means that the statement proven by the ZAP really lies in $\NP\cap \coNP$. 

\para{The Super-Complement Languages.} To obtain a compact construction, the signature size should be sub-polynomial on the ring size. In particular, the size of the ZAP proof should be sub-polynomial on the ring size. To capture this property, \cite{C:CGHKLMPS21} abstracts out the following notion of {\em super-complement languages}, which can be interpreted as a generalization of $\NP\cap\coNP$ where an (augmented) complement langauge is specified explictly. As it will become clear in \Cref{sec:building-blocks:language}, this helps to split the ring and the other sub-polynomial-size part in a signature. In the following, we follow the \cite{C:CGHKLMPS21} framework to present the definition of super-complement languages and ZAPs for them. Then, We will instantiate in \Cref{sec:building-blocks:language} a concrete super-complement language used in our ring signature construction.

\begin{definition}[Super-Complement \cite{C:CGHKLMPS21}]\label{def:super-complement-language}
    Let $(L, \widetilde{L})$ be two $\NP$ languages where the elements of $\widetilde{L}$ are represented as pairs of bit strings. We say $\widetilde{L}$ is a \emph{super-complement} of $L$, if 
    $\widetilde{L} \subseteq (\bits^*\setminus L) \times \bits^*$. 
    I.e., $\widetilde{L}$ is a super complement of $L$ if for any $x= (x_1,x_2)$, $x \in \widetilde{L} \Rightarrow x_1 \not \in L$.   
\end{definition}

We now define ZAPs for super-complement languages consisting of pairs of the form $(L,\widetilde{L})$. Notice that, while the complement of $L$ might not be in $\NP$, it must hold that $\widetilde{L} \in \NP$. The language $\widetilde{L}$ is used to define the soundness property. Namely, producing a proof for a statement $x = (x_1, x_2) \in \widetilde{L}$, should be hard. We also use the fact that $\widetilde{L} \in \NP$ to mildly strengthen the soundness property. In more detail, instead of having selective soundness where the statement $x \in \widetilde{L}$ is fixed in advance, we now fix a non-witness $\widetilde{w}$ and let the statement $x$ be adaptively chosen by the malicious prover from all statements which have $\widetilde{w}$ as a witness to their membership in $\widetilde{L}$. 



\begin{definition}[ZAPs for Super-Complement Languages \cite{C:CGHKLMPS21}]
    \label{def:generalizedzap-interface}
    Let $L,\widetilde{L} \in \NP$ s.t.\ $\widetilde{L}$ is a super-complement of $L$. Let $R$ and $\widetilde{R}$ denote the $\NP$ relations corresponding to $L$ and $\widetilde{L}$ respectively. Let $\{C_{n,\ell}\}_{n,\ell}$ and $\{\widetilde{C}_{\tilde{n},\tilde{\ell}}\}_{\tilde{n},\tilde{\ell} }$ be the $\NP$ verification circuits for $L$ and $\widetilde{L}$ respectively. Let $\widetilde{d} = \widetilde{d}(\tilde{n},\tilde{\ell})$  be the depth of $\widetilde{C}_{n,\ell}$. A \emph{compact relaxed ZAP} for~$L,\widetilde{L}$
    is a tuple of PPT algorithms
    $(\algo{V}, \algo{P}, \algo{Verify})$ having the following
    interfaces (where $1^{n}, 1^{\lambda}$ are implicit inputs to
    $\algo{P}$, $\algo{Verify}$):
    \begin{itemize}
        \item 
        {\bf $\algo{V}(1^{\lambda}, 1^n,1^{\widetilde{\ell}}, 1^{\widetilde{D}})$:} 
        On input a security parameter $\lambda$, 
        statement length~$n$ for $L$, 
        witness length $\widetilde{\ell}$ for $\widetilde{L}$, 
        and $\NP$ verifier circuit depth upper-bound $\widetilde{D}$ for $\widetilde{L}$, output a first message
        $\rho$.
        \item 
        {\bf $\algo{P}\big(\rho,x = (x_1,x_2),w\big)$:} On input a string~$\rho$, a statement $(x_1 \in \bits^{n},x_2)$, and a witness $w$ such that $(x_1,w) \in R$, output a proof~$\pi$.
        \item 
        {\bf $\algo{Verify}\big(\rho,x = (x_1,x_2),\pi\big)$:} On input a string $\rho$, a
        statement $x$, and a proof $\pi$, output either 1 (accepting) or 0 (rejecting).
    \end{itemize}
The following requirements are satisfied:
    \begin{enumerate}
        \item {\bf Completeness:} For every $(x_1,w) \in L$, every $x_2 \in \bits^*$,
        every $\widetilde{\ell} \in \Naturals$, 
        every $\widetilde{D} \ge \widetilde{d}(\abs{x_1} + \abs{x_2},\widetilde{\ell})$, 
        and every
        $\lambda \in \Naturals$, \[\Pr[\algo{Verify}\big(\rho,x = (x_1,x_2),\pi\big)=1 ] = 1, \]  
        where
        $\rho \gets \algo{V}(1^{\lambda}, 1^{\abs{x_1}},1^{\widetilde{\ell}}, 1^{\widetilde{D}})$ and
        $\pi \gets \algo{P}(\rho,x,w)$.
        
        \item {\bf Public coin:}
            $\algo{V}(1^{\lambda}, 1^n,1^{\widetilde{\ell}}, 1^{\widetilde{D}})$ simply outputs a uniformly
            random string.
        
        \item \label{item:def:zap:soundness}
        {\bf Selective non-witness adaptive-statement soundness:} 
        For any non-uniform QPT machine $P^*_{\lambda}$, any $n,\widetilde{D} \in \Naturals$, and any non-witness $\widetilde{w} \in \bits^{*}$, the following holds
        \begin{equation*}
            \Pr[
            \begin{array}{l}
            \rho \gets \algo{V}(1^{\lambda}, 1^{n},1^{\abs{\widetilde{w}}}, 1^{\widetilde{D}});\\
            \big(x = (x_1,x_2),\pi^*\big) \gets P^*_{\lambda}(\rho)
            \end{array}: 
            \begin{array}{l}
                \algo{Verify}(\rho,x,\pi^*) = 1 ~\wedge\\
                \widetilde{D} \ge \widetilde{d}(\abs{x}, \abs{\widetilde{w}}) ~\wedge~ (x,\widetilde{w}) \in \widetilde{R}
            \end{array} ] \le \negl(\SecPar).
        \end{equation*}
        
%       \item {\bf Witness indistinguishiability}: for every two witnesses $w_1, w_2$ such that $(x,w_1) \in \mathcal{R}$ and $(x,w_2) \in \mathcal{R}$, and every non-uniform polynomial-size ``cheating''
%       verifier $V^{*}$  the
%       following two distribution ensembles are indistinguishable:
%       \begin{equation}
%       \set{ \mathcal{S}(1^{\lambda},x) }_{\lambda} \statind \set{
%           (\rho, \algo{Prover}(\rho,x,w)) : \rho \gets
%           \algo{Setup}(1^{\abs{x}},1^{\lambda})}_{\lambda} \; .
%       \end{equation}
        
        \item {\bf Statistical witness indistinguishability:} For every (possibly unbounded) ``cheating''
        verifier $V^{*}=(V^{*}_{1}, V^{*}_{2})$ and every $n,\widetilde{\ell},\widetilde{D} \in \Naturals$, the
        probabilities
        \[ \Pr[V^{*}_{2}(\rho,x,\pi,\zeta)=1 ~\wedge~ (x,w) \in  \mathcal{R} ~\wedge~ (x,w')  \in \mathcal{R} ] \] in the
        following two experiments differ only by $\negl(\lambda)$:
        \begin{itemize}
            \item in experiment 1,
            $(\rho,x,w,w',\zeta) \gets
            V^{*}_{1}(1^{\lambda}, 1^{n},1^{\widetilde{\ell}}, 1^{\widetilde{D}}), \pi \gets \algo{P}(\rho,x,w)$;
            
                \item in experiment 2,
            $(\rho,x,w,w',\zeta) \gets
            V^{*}_{1}(1^{\lambda}, 1^{n},1^{\widetilde{\ell}}, 1^{\widetilde{D}}), \pi \gets \algo{P}(\rho,x,w')$.               
        \end{itemize}  
    \item {\bf Compactness (Optional):} The ZAP is {\em compact} if the size of the proof $\pi$ (output by $\algo{P}$) is a fixed polynomial in $n$, $\widetilde{\ell}$, $\widetilde{D}$, $|C|$, and $\lambda$. In particular, it is independent of the size of $\widetilde{C}$ and $x_2$.   
    \end{enumerate}
\end{definition}

\cite{C:CGHKLMPS21} constructs such an ZAP assuming LWE. We remark that \cite{C:CGHKLMPS21} only claims soundness (\Cref{item:def:zap:soundness}) against non-uniform PPT adversaries. But it is straightforward to see  that their proof for soundness also works against non-uniform QPT adversaries assuming the quantum hardness of LWE.
\begin{lemma}[\cite{C:CGHKLMPS21}]\label{lem:ZAP:from:QLWE}
Assuming QLWE, there exist compact ZAPs (as per \Cref{def:generalizedzap-interface}) for any super-complement language (as per \Cref{def:super-complement-language}).
\end{lemma}




\subsection{Construction}
Our construction, shown in \Cref{constr:pq:ring-sig}, relies on the following building blocks. Note that except for \Cref{item:RS:building-block}, which is a information-theoretical primitive, all of the others can be constructed assuming QLWE.
\begin{enumerate}
    \item \label{item:RS:building-block}
    Pair-wise independent functions;
    
    \item 
    An blind-unforgeable signature scheme $\algo{Sig}$ satisfying \Cref{def:classical-BU-sig}; 
    
    \item 
    A lossy public key encryption scheme $\LE$ satisfying \Cref{def:special-LE};
   
    \item 
    A somewhere perfectly binding hash function $\algo{SPB}$ satisfying \Cref{def:SPB-hash};
    
    \item 
    A compact ZAP scheme $\algo{ZAP}$ satisfying \Cref{def:generalizedzap-interface}.
\end{enumerate}
We remark that the $\RS.\Sign$ algorithm runs $\ZAP$ on a special super-complement language $(L, \tilde{L})$, whose definition will appear after the construction in \Cref{sec:building-blocks:language}. Such an arrangement is because we find that the language $(L, \tilde{L})$ will become easier to understand once the reader has the big picture of \Cref{constr:pq:ring-sig}.

% Before present the construction, we need to take one more detour to specify the super-complement language on which the signing algorithm run $\ZAP$.




\begin{xiaoenv}{Explain the difference with \cite{C:CGHKLMPS21}:}
Explain the difference with \cite{C:CGHKLMPS21}:
\begin{itemize}
\item
 we replace PKE with $\LE$ to obtain post-quantum anonymity.
\item
    the ZAP must be statistical WI, while \cite{C:CGHKLMPS21} only needs computational WI\footnote{Although \cite{C:CGHKLMPS21} builds and employs a ZAP with statistical WI in their ring signature, computational WI already suffices for their security proof.}.
 \item
 We need pair-wise independent hash function to invoke Zhandry's lemma.
 \item
 Need to make the $\SPB.\Gen(1^\secpar, M, i)$ use a universal upper bound for database size, independent of $|\Ring|$. Thus, the \SPB keys are generated only once, instead of one time for each $\Ring$'s in superposition. I think we can use $M$ as the universal upper bound. But we need to make sure that a $\SPB.\Gen(1^\secpar, M, i)$ can be used to hash $\Ring$ with $|\Ring| \le M$. I think this could be done by padding $\Ring$ with dummies to size $M$. Note that the signature size scales with $\log(M)$.
 \item
 The $\algo{Sig}$ in our construction should be BU secure.
 \item
 I need to sign it as $\algo{Sig}.\Sign(sk, \Ring \| m)$, where $\Sig$ is a short signature scheme.
\end{itemize}
\end{xiaoenv}

\begin{construction}
\label{constr:pq:ring-sig}
Let $\widetilde{D} = \widetilde{D}(\lambda, N)$ %\footnote{We emphasis that $\tilde{D}$ is poly-logarithmic on $N$. See the definition of $\tilde{L}$ in \Cref{eq:def:language:L-tilde}.} 
be the maximum depth of the $\algo{NP}$ verifier circuit for language $\widetilde{L}$ restricted to statements where the the ring has at most $N$ members, and the security parameter for $\algo{SPB}$, \Sig, and $\algo{LE}$ is $\lambda$. Let $n = n(\lambda,\log N)$ denote the maximum size of the statements of language $L$ where the ring has at most $N$ members and the security parameter is $\lambda$. Recall that for security parameter $\lambda$, secret keys in $\LE$ have size $\widetilde{\ell} = \ell_{\sk}(\lambda)$. We now describe our ring signature construction: 

\subpara{Key Generation Algorithm $\algo{Gen}(1^\lambda,N)$:} 
    \begin{itemize}[topsep=0.2em,itemsep=0em]
        \item sample signing/verification key pair: $(vk,sk) \gets \algo{Sig.Gen}(1^\lambda)$;
        \item sample obliviously an injective public key of $\algo{LE}$: $pk \gets \LE.\KSam^\ls(1^\secpar)$;     
        \item compute the first message $\rho \leftarrow \algo{ZAP.V}(1^\lambda,1^n,1^{\widetilde{\ell}},1^{\widetilde{D}})$ for the relaxed ZAP scheme;
        \item output the verification key $\VK\coloneqq (vk,pk,\rho)$ and signing key $\SK\coloneqq (sk,vk,pk,\rho)$.
    \end{itemize}

\subpara{Signing Algorithm $\algo{Sign}(\SK,\Ring, m)$:}
    \begin{itemize}[topsep=0.2em,itemsep=0em]
    	\item parse $\Ring = (\VK_1,\dots,\VK_{\ell})$; and parse $\SK=(sk,vk,pk,\rho)$;
        \item compute $\sigma \gets \algo{Sig.Sign}(sk,\Ring\|m)$; \xiao{this could lead a problem to define $L$ and $\tilde{L}$.}
        \item let $\VK \coloneqq \VK_i \in R$ be the verification key corresponding to $\SK$; 
        \item let $M = 2^{\log^2\secpar}$ (see \Cref{rmk:SPB:setting-M}); sample independently two pairs of hash keys:\vspace{-0.7em}
         $$(hk_1,shk_1) \gets \algo{SPB.Gen}(1^\lambda,M,i),~(hk_2,shk_2) \gets \algo{SPB.Gen}(1^\lambda,M,i),\vspace{-0.7em}$$ and compute $h_1 \gets \algo{SPB.Hash}(hk_1,\Ring)$ and $h_2 \gets \algo{SPB.Hash}(hk_2,\Ring)$; 

        \item compute the opening $\tau_1 \gets \algo{SPB.Open}(hk_1,shk_1,\Ring,i)$ to position $i$;
        
        \item 
        sample tow pairwise-independent functions $\PI_1$ and $\PI_2$, and compute
         \vspace{-0.8em}$$r_{c_1} = \PI_1(\Ring\|m), ~~r_{c_2} = \PI_2(\Ring\|m).\vspace{-0.8em}$$
        \item compute $c_1 \gets \algo{LE.Enc}(pk,(\sigma,vk);r_{c_1})$ and  $c_2 \gets \algo{LE.Enc}(pk,0^{|\sigma|+|vk|};r_{c_2})$;
        
        \item 
        let $\VK_1 = (vk_1,pk_1,\rho_1)$ denote the lexicographically smallest member of $\Ring$ (as a string; note that this is necessarily unique); 
        
        \item 
        fix statement $x_1=(m,c_1,c_2,hk_1,hk_2,h_1,h_2)$,  witness $w=(vk,pk,i,\tau_1,\sigma,r_{c_1})$, and statement $x_2 = \Ring$. We remark that these statements and witness correspond to a super-complement language $(L, \tilde{L})$ that will be defined in \Cref{sec:building-blocks:language}. Looking ahead, $x_1$ with witness $w$ is a statement in the $L$ defined in \Cref{eq:def:language:L}; $(x_1, x_2)$ constitute a statement that is {\em not} in the $\tilde{L}$ defined in \Cref{eq:def:language:L-tilde}. 
        \item sample another pairwise-independent function $\PI_3$ and compute $r_\pi = \PI_3(\Ring\|m)$;
        \item compute $\pi \gets \algo{ZAP.P}(\rho_1,x=(x_1,x_2),w; r_\pi)$;
        \item output $\Sigma = (c_1,hk_1,c_2,hk_2,\pi)$.
    \end{itemize}

\subpara{Verification Algorithm $\algo{Verify}(\Ring,m, \Sigma)$:}
    \begin{itemize}[topsep=0.2em,itemsep=0em]
        \item identify the lexicographically smallest verification key $\VK_1$ in $\Ring$;
        \item compute $h'_1 = \algo{SPB.Hash}(hk_1,\Ring)$ and $h'_2 = \algo{SPB.Hash}(hk_2,\Ring)$;
        \item fix $x_1=(m,c_1,c_2,hk_1,hk_2,h'_1,h'_2)$ and $x_2 = \Ring$;  read $\rho_1$ from $\VK_1$; 
        \item compute and output $\algo{ZAP}.\algo{Verify}(\rho_1,x,\pi)$.
\end{itemize}
\end{construction}

\subsubsection{The Super-Complement Language Proven by the ZAP}
\label{sec:building-blocks:language}
We now define the super-complement language $(L, \widetilde{L})$ used in \Cref{constr:pq:ring-sig}. It is similar to the $(L, \tilde{L})$ defined in \cite[Section 5]{C:CGHKLMPS21}, but with necessary modifications to accommodate \Cref{constr:pq:ring-sig}.  

For a statement of the form $y_1 = (m,c,hk,h)$ and witness $w =  \big(\mathsf{VK}=(vk,pk,\rho),i,\tau,\sigma,r_c \big)$, define relations $R_1,R_2$ and $R_3$ as follows:
\begin{align*}
    (y_1,w) \in R_1 & ~\Leftrightarrow~ \algo{SPB.Verify}(hk,h,i,\mathsf{VK},\tau)=1\\
    (y_1,w) \in R_2 &  ~\Leftrightarrow~ \algo{LE.Enc}\big(pk,(\sigma,vk);r_c\big) = c\\
    (y_1,w) \in R_3 & ~\Leftrightarrow~ \algo{Sig.Verify}(vk,m,\sigma)=1 ~~~~\red{(\Ring\|m)???}
\end{align*}
Next, define the relation $R'$ as  $R'\coloneqq R_1\cap R_2 \cap R_3$. Let $L'$ be the language corresponding to $R'$. Define language $L$ as 
\begin{equation}\label{eq:def:language:L}
L \coloneqq \bigg\{(m,c_1,c_2,hk_1,hk_2,h_1,h_2) ~\bigg|~ 
\begin{array}{l}
(m,c_1,hk_1,h_1) \in L' ~\vee \\
(m,c_2,hk_2,h_2) \in L' 
\end{array}\bigg\}.
\end{equation}

Now, we define another language $\widetilde{L}$ and prove that it is a super-complement of $L$ in \Cref{lemma:ring-sig:complement}. Let $x_2 \coloneqq \algo{R}$ where $\Ring = (\algo{VK_1,\dots,VK_\ell})$. Let $y \coloneqq (y_1,x_2)$, and $\widetilde{w} \coloneqq s$. Define the following relations:
\begin{align}
    (y,\widetilde{w})\in R_4 & ~\Leftrightarrow~ \big(\forall j \in [\ell]:  \algo{LE.Valid}(pk_j,s)=1\big) \wedge \big(h =  \algo{SPB.Hash}(hk,\algo{R})\big) \label{def:relation:R4}\\
    (y,\widetilde{w})\in R_5 & ~\Leftrightarrow~ 
    \left\{
        \begin{array}{l}
        \algo{LE.Dec}(s,c) = (\sigma,vk) \wedge \algo{Sig.Verify}(vk, m, \sigma)=1 ~\wedge \\
        \exists\algo{VK} \in \mathsf{R}: \algo{VK} = (vk,pk,\rho) \text{ for some } pk \text{ and } \rho
        \end{array} 
    \right. \label{def:relation:R5}
\end{align}
where, for each $j \in [\ell]$,  $\algo{VK}_j = (vk_j, pk_j, \rho_j)$.  Let $L_4$ and $L_5$ be the languages corresponding to $R_4$ and $R_5$, respectively. Define further the relation $\widehat{R}$ according to $\widehat{R} \coloneqq R_4 \setminus R_5$, and let $\widehat{L}$ be the corresponding language. Define $\tilde{L}$ as follows:
\begin{equation}\label{eq:def:language:L-tilde}
\widetilde{L} \coloneqq \bigg\{(
\underbrace{m,c_1,c_2,hk_1,hk_2,h_1,h_2}_{\coloneqq x_1},\underbrace{\mathsf{R}{\color{white})}}_{\coloneqq x_2}) ~\bigg|~ 
\begin{array}{l}
(m,c_1,hk_1,h_1,\algo{R}) \in \widehat{L}  ~\wedge \\
(m,c_2,hk_2,h_2,\algo{R}) \in \widehat{L}
\end{array}
\bigg\}.
\end{equation} 
The next claim shows that $\tilde{L}$ is indeed the super-complement of $L$.
\begin{MyClaim}
    \label{lemma:ring-sig:complement}
    If $\algo{SPB}$ is somewhere perfectly binding and $\LE$ is complete (\Cref{item:def:LE:completeness}), then the $\widetilde{L}$  (\Cref{eq:def:language:L-tilde}) is a super-complement of $L$ (\Cref{eq:def:language:L}).
\end{MyClaim}
\begin{proof}
It is straightforward to see that $L, \tilde{L} \in \NP$. To prove this lemma, we need to show that for any statement $x$ of the following form 
\begin{equation}\label{eq:ring-sig:complement:statement:x}
x =  \big(x_1 =(m,c_1,c_2,hk_1,hk_2,h_1,h_2),x_2 = \algo{R}\big),
\end{equation}
it holds that $x \in \tilde{L} \Rightarrow x_1 \notin L$ (see \Cref{def:super-complement-language}). In the following, we finish the proof by showing the contrapositive: $x_1 \in L \Rightarrow x\notin \tilde{L}$. 

For any $x$ as in \Cref{eq:ring-sig:complement:statement:x}, we define 
$$y_1 \coloneqq (m,c_1,hk_1,h_1) ~\text{and}~ y'_1 \coloneqq (m,c_2,hk_2,h_2).$$
To prove ``$x_1 \in L \Rightarrow x\notin \tilde{L}$'', it suffices to show that the following \Cref{eq:ring-sig:complement:expression1,eq:ring-sig:complement:expression2} hold for every $w= (\algo{VK}= (vk,pk,\rho),i,\tau,\sigma,r_c)$ and every $\widetilde{w} = s$:
\begin{align}
&(y_1,w) \in R' \wedge \big((y_1,x_2),\widetilde{w}\big) \in R_4 ~\Rightarrow~ \big((y_1,x_2), \widetilde{w} \big) \in R_5  \label[Expression]{eq:ring-sig:complement:expression1}\\
&(y_1',w) \in R' \land \big((y_1',x_2),\widetilde{w}\big) \in R_4 ~\Rightarrow~ \big((y_1',x_2), \widetilde{w} \big) \in R_5. \label[Expression]{eq:ring-sig:complement:expression2}
\end{align}

We first prove \Cref{eq:ring-sig:complement:expression1}. If $(y_1,w) \in R_1$ and $\big((y_1,x_2),\widetilde{w}\big) \in R_4$, then, by the somewhere perfectly binding of $\algo{SPB}$, we have $\algo{VK} \in \algo{R}$. Now, notice that by the completeness property (\Cref{item:def:LE:completeness}) of $\algo{LE}$, since $\algo{LE.Valid}(pk,s) = 1$, if  $(y_1,w) \in R_2 \cap R_3$,   then $(y_1,\widetilde{w}) \in R_5$. 

\Cref{eq:ring-sig:complement:expression2} can be proven similarly. This finish the proof of \Cref{lemma:ring-sig:complement}.
\end{proof}

\subsection{Proving Post-Quantum Security}
We now prove that \Cref{constr:pq:ring-sig} is a post-quantum secure post-quantum ring signature satisfying \Cref{def:pq:ring-signatures}. Its completeness follows straightforwardly from the completeness of $\algo{SPB}$, $\ZAP$, and $\algo{Sig}$. For compactness, notice that the only steps in \Cref{constr:pq:ring-sig} that could possibly depend on the ring size is the \ZAP proof and the $\Sig.\Sign(sk, \Ring\| m)$.

, the compactness of \Cref{constr:pq:ring-sig} follows from the compactness of $\ZAP$. Next, we prove the post-quantum anonymity and unforgeability in \Cref{sec:prove:pq:anonymity} and \Cref{sec:prove:pq:blind-unforgeability}, respectively.





==> sections/tech_overview.tex <==
%!TEX root=../main.tex
\section{Technical Overview}

\red{tech overview goes here...}


